mRSC: Multi-dimensional Robust Synthetic Control

When evaluating the impact of a policy on a metric of interest, it may not be possible to conduct a randomized control trial. In settings where only observational data is available, Synthetic Control (SC) methods provide a popular data-driven approach to estimate a "synthetic" control by combining measurements of "similar" units (donors). Recently, Robust SC (RSC) was proposed as a generalization of SC to overcome the challenges of missing data high levels of noise, while removing the reliance on domain knowledge for selecting donors. However, SC, RSC, and their variants, suffer from poor estimation when the pre-intervention period is too short. As the main contribution, we propose a generalization of unidimensional RSC to multi-dimensional RSC, mRSC. Our proposed mechanism incorporates multiple metrics to estimate a synthetic control, thus overcoming the challenge of poor inference from limited pre-intervention data. We show that the mRSC algorithm with $K$ metrics leads to a consistent estimator of the synthetic control for the target unit under any metric. Our finite-sample analysis suggests that the prediction error decays to zero at a rate faster than the RSC algorithm by a factor of $K$ and $\sqrt{K}$ for the training and testing periods (pre- and post-intervention), respectively. Additionally, we provide a diagnostic test that evaluates the utility of including additional metrics. Moreover, we introduce a mechanism to validate the performance of mRSC: time series prediction. That is, we propose a method to predict the future evolution of a time series based on limited data when the notion of time is relative and not absolute, i.e., we have access to a donor pool that has undergone the desired future evolution. Finally, we conduct experimentation to establish the efficacy of mRSC on synthetic data and two real-world case studies (retail and Cricket).

==> content/algorithm.tex <==
% Algorithm
\section{Algorithm} \label{sec:algorithm}

\subsection{Inputs.}
The multi-Robust Synthetic Control (mRSC) algorithm takes several inputs. For simplicity, we assume that there exist {\em two} metrics of interest. The same arguments can naturally be extended to any number of metrics of interest. However, we choose two to better illustrate the algorithm. The two metrics are represented by $N \text{(donor units)} \times T \text{(periods)}$ observation matrices denoted by $\bA^1$ and $\bA^2$. The corresponding unobserved mean matrices are denoted by $\bM^1$ and $\bM^2$. The intervention, i.e. the period after which we want to estimate the forecasts, is denoted by $T_0 < T$. Therefore, the data used for training is represented by $\bA^{1-}$ and $\bA^{1-}$ which are subsets of the observation matrices but for column indices in $[1, ... , T_0]$. The post-intervention matrices are similarly denoted by  $\bA^{1+}$ and $\bA^{1+}$ which are subsets of the observation matrices but for column indices in $[T_0+1, ... , T]$. The unobserved mean matrices $\bM^{1-}$, $\bM^{2-}$, $\bM^{1+}$ and $\bM^{2+}$ are defined similarly. Our unit of interest is the denoted by $y^1_1$ and $y^2_1$. Given that we are interested in estimating the post-intervention future of this unit of interest, both $y^1$ and $y^2$ are of dimension $1 \times T_0$. 

The pre-intervention observation matrices are row-concatenated in to a combined observation matrix, $\bY^-$, which has dimensions $N \times 2T_0$. Specifically, $\bY^- = [\bA^{1-} \quad \bA^{2-}]$. Similarly, we refer to the row-combined but unobserved mean matrix by $\bM^- = [\bM^{1-} \quad \bM^{2-}]$. The post-intervention observation matrices are similarly row-concatenated and denoted by $\bY^+ = [\bA^{1+} \quad \bA^{2+}]$ but have dimensions $N \times 2(T - T_0)$. Finally, the pre-intervention observations from the unit of interest are denoted by $y^- = [y^1 \quad y^2]$. 

Given that the mRSC algorithm is a generalization of the Robust Synthetic Control (RSC) algorithm, it uses the same hyper-parameters: (1) a thresholding hyperparameter $\mu \geq 0$, which helps threshold the singular value spectrum of the observation matrix and effectively serves as a knob to effectively trade-off between the bias and variance of the estimator \cite{rsc1}, and (2) a regularization hyper-pameter $\eta \ge 0$ that controls the model complexity \cite{rsc1}. There is one additional parameter used by the mRSC algorithm: (3) a loss-function weighting between the two metrics, $\delta_1, \delta_2$. This parameter helps generalize the regularized OLS regression step in the RSC algorithm \cite{rsc1} to a regularized Weighted Least Squares (WLS) step. If both metrics are of the same order of magnitude and importance, then $\delta_1 = \delta_2$. However, a different weighting can help denote the relative importance (or correction) between the two metrics. Effectively, this helps creating a diagonal matrix, $\Delta = diag([\frac{1}{\sqrt{\delta_1}}, ... ,  \frac{1}{\sqrt{\delta_2}}, ...])$, which can pre-multiply the observation matrix, $\bM$ and unit of interest, $y$. Similar to \cite{rsc1}, these parameters can be chosen via several data-driven techniques, e.g. cross-validation.

\subsection{Missing Data}
To further simplify the exposition of the mRSC algorithm, we assume no missing data. If we encounter missing data in the problem, it can be modeled similar to the RSC algorithm with a probability of observation $p$. It is trivial to extend the mRSC algorithm to incorporate missing data similar to the vanilla RSC algorithm.

%We begin by exploring the intuition behind our proposed two-step algorithm: (1) \textit{de-noising the data:} since the singular values of our observation matrix, $\bX = [X_{it}]_{2 \le i \le N, t \in [T]}$, encode both signal and noise, we aim to discover a low rank approximation of $\bX$ that only incorporates the singular values associated with useful information; simultaneously, this procedure will naturally impute any missing observations. We note that this procedure is similar to the algorithm proposed in \cite{usvt}. (2) \textit{learning $\beta^*$:} using the pre-intervention portion of the de-noised matrix, we learn the linear relationship between the treatment unit and the donor pool prior to estimating the post-intervention counterfactual outcomes. Since our objective is to produce accurate predictions, it is not obvious why the synthetic treatment unit should be a convex combination of its donor pool as assumed in \cite{abadie1, abadie3, abadie4}. In fact, one can reasonably expect that the treatment unit and some of the donor units may exhibit negative correlations with one another. In light of this intuition, we learn the optimal set of weights via linear regression, allowing for both positive and negative elements. 

%Finally, (3) \textit{paired-sample hypothesis test:} we obtain a t-statistic, $\tau$, for a paired-sample hypothesis test and determine if it is above/below a significance threshold to conclude that the two post-intervention samples, i.e. actual and predicted counter-factual, are statistically indistinguishable (null hypothesis) or not (alternate hypothesis). Note that the paired-sample t-test assumes independence, which is satisfied by our model where the errors are assumed to be independent across time and location. \\

\subsection{Robust Multi-Metric Algorithm.} \label{sec:robust_algo}
%We present the details of our robust method in Algorithm \ref{euclid} below. The algorithm utilizes two hyperparameters: (1) a thresholding hyperparameter $\mu \geq 0$, which serves as a knob to effectively trade-off between the bias and variance of the estimator, and (2) a regularization hyperameter $\eta \ge 0$ that controls the model complexity. We discuss the procedure for determining the hyperparameters in Section \ref{sec:fineprint}. To simplify the exposition, we assume the entries of $\bX$ are bounded by one in absolute value, i.e. $ \abs{X_{it} } \leq 1$.

%\noindent
%\textit{Note}: To simplify the exposition, we assume the entries of $\bX$ are bounded by one in absolute value, i.e. $ \abs{X_{it} } \leq 1$. 

Using the inputs, we are now ready to describe the mRSC algorithm. Recall that the goal is to estimate the future of the unit of interest. This estimated forecast is denoted by $\hat{m}_1^+$. Given that we have two metrics of interest, the first half of the estimate belong to first metric and the second half to the second metric.
\begin{algorithm}
\caption{Multi Robust Synthetic Control (mRSC)}\label{euclid}
\noindent \\

{\bf Step 1. De-noising: singular value thresholding.} \\
\begin{enumerate}
	\item Weight the observation matrices and unit of interest by the corresponding weights, represented by the diagonal matrix $\Delta$:
	\begin{align}
		\bY^- &=  \bY^- \Delta, \\
		y^- &=   y^- \Delta
	\end{align}
	\item Compute the singular value decomposition of $\bY^{-}$:
	\begin{align}
		\bY^-  = \sum_{i=1}^{N} s_i u_i v_i^T.
	\end{align}

	\item Let $S = \{ i : s_i \geq \mu\}$ be the set of singular values above the threshold $\mu$.

	\item Define the estimator of $\bM^-$ as 
	\begin{align} \label{eq:p_hat}
		\bhM^- & = \sum_{i \in S} s_i u_i v_i^T,
	\end{align}
\end{enumerate} 

\noindent \\
{\bf Step 2. Regularized (Weighted) Least Squares.} \\

\begin{enumerate}
	\item For any $\eta \ge 0$, let
	\begin{align} 
		\hat{\beta}(\eta) &= \argmin_{v \in \mathbb{R}^{N}} \norm{y^{-} - (\bhM^{-})^T v}^2 + \eta \norm{v}^2 \label{eq:ls}.
	\end{align}
	
	\item Define the estimated (counterfactual) means for the treatment unit as 
	\begin{align}
		\hat{m}_1^+ & = \bY^{+T} \hat{\beta}(\eta).
	\end{align}
\end{enumerate} 
\end{algorithm}

Finally, we note that all the features of the vanilla RSC algorithm extend naturally to the mRSC algorithm (see Section 3.4 of \cite{rsc1}). Specifically, all properties of RSC regarding solution interpretability, scalability, low-rank hypotheses and independence from using covariate information are also features of the mRSC algorithm. Effectively, the mRSC algorithm is a generalization of the RSC algorithm in that it incorporates learning based on multiple metrics of interest. 
























==> content/introduction__Muhammad_Amjad_s_conflicted_copy_2019-02-18_.tex <==
\section{Introduction} \label{sec:intro}

Quantifying the causal statistical effect of interventions is a problem of interest across a wide array of domains. 
From policy to engineering to medicine, estimating the effect of an intervention is critical to innovation and understanding 
existing systems. In any setting, with or without an intervention, we only get to observe one set of outcomes. In casual 
analysis, the fundamental problem is that of estimating what wasn't observed, the {\em counterfactual}. 
%
%
% i.e. another set of outcomes. Specifically, when evaluating the effect of a treatment on a unit of interest, we observe the effects of that treatment. In order to quantify the effect as significant (or not), the counterfactual must be estimated, i.e. the unobserved outcomes that {\em would have} happened {\em without} the intervention. Our focus is on this problem of estimating the counterfactual. 
% 
% Specifically, given an arbitrary intervention point, our problem of interest is to estimate what would have happened if there was no {\em actual} intervention and things continued in the same vein as before the arbitrarily chosen evaluation point.

%We consider the setup of observational studies where experimental studies are not feasible to estimate the {\em counterfactual}. 
In order to estimate the counterfactual, observational studies rely on the identification (or estimation) of a {\em control} unit. This can be done by experts or via techniques such as {\em matching} the unit of interest to other units (called {\em donors}) on covariate features or propensity scores (see \cite{rubin1973, rosenbaum1983}) etc. A popular data-driven approach to estimating the control unit is known as the Synthetic Control Method (SCM)  \cite{abadie1, abadie2, abadie3}. SCM assigns convex weights to the donors such that the resulting {\em synthetic} unit most closely matches the unit of interest, according to a chosen metric of interest. A generalization of this approach known as the Robust Synthetic Control (RSC) \cite{rsc1} removes the convexity constraint and guarantees a consistent estimator which is robust to missing data and noise. 

While the SCM, its many variants and the RSC have been shown to have attractive properties, they all suffer for poor estimation when 
the amount of training data, i.e. the length of the pre-intervention period, is small. In many of these scenarios with little pre-intervention data, there may be other data available which is related to the type of data (or metric) of interest. For example, we might be interested in crime-rate and might also have median household income and high-school graduation rate data available. Therefore, one remedy to 
the limited pre-intervention data is to utilize data from multiple metrics. 

%
%\subsection{Problem Statement}
%Given a unit of interest say unit $1$, $N-1$ donor units and data for $K > 1$ metrics observed for $T_0$ time periods (for all $N$ units), 
%the problem considered in this work is that of estimating the mean {\em synthetic} control unit for the unit of interest. 
%
%Additionally, it is our goal to use the synthetic control to estimate, or {\em forecast}, the mean counterfactual for the unit of interest (for all $K$ metrics) from time periods $(T_0, T]$.
%
%%\todo[inline]{We need to clarify here that our interest in this paper is not the counterfactual for analyzing impact of an actual intervention, rather it is for timeseries prediction}
%
%Here we note that for most of the experimentation in this work we use arbitrary {\em interventions} which should have no statistical effect. Our goal is to use the observed data to estimate the mean effects {\em without} any changes. Therefore, we are only concerned with the problems of estimation of the control unit and its forecasts (counterfactual). 

\subsection{Contributions}

As the main contribution of this work, we propose a generalization of unidimensional RSC to multidimensional Robust Synthetic Control (mRSC). In the process we address the challenge of poor estimation of the counterfactual 
due to limited pre-intervention data since the mRSC incorporates multiple-types of data in a principled manner.
We show that the mRSC method is a natural consequence of the popular factor model. Through this connection, we provide a falsifiability test for mRSC in a data-driven manner. In particular, we establish that if test is passed, then mRSC can be expected to produce a consistent estimation of the mean unit of interest (for all metrics) in the pre- and post-intervention periods. Further, the accuracy of estimating control using mRSC improves with respect to the RSC with increasing number of different types of relevant data. Specifically, the Mean Squared Error (MSE) is decreased by a factor of $K$ and $\sqrt{K}$ for the pre- and post-intervention estimates. All other properties of the RSC algorithm, namely robustness to missing data and noise, carry over. Finally, we conduct extensive experimentation to establish the efficacy of this generalized method in comparison to the RSC algorithm via synthetically generated datasets and two real-world case-studies: product sales in retail and score trajectory forecasting in game of Cricket. Next, we summarize these contributions in more detail.

\medskip
\noindent {\bf Model.} We consider a natural generalization of the factor (or latent variable) model considered in the literature cf. \cite{rsc1} where the measurement associated with a given unit, at a given time for a given metric is a function of features associated with the unit, time and the metric. A special case of such models, the linear factor models, are the {\em bread and butter} models within the Econometrics literature and assumed in \cite{abadie1, abadie2, abadie3}. We argue that  as long as function is Lipschitz and the features belong to a compact domain, the resulting factor model can be well approximated by low-rank 3-order tensor with three dimensions of the tensor corresponding to the unit, time and metric, respectively. Therefore, for simplicity of exposition, we focus on setup where the underlying model is indeed a low-rank 3-order tensor. The observations are noisy version of the ground truth 3-order low-rank tensor with potentially missing values. These include pre-intervention data for all units and metrics, while post-intervention data only for the ``donor'' units. The goal is to estimate the ``synthetic control'' using all donor units and all the metrics in the pre-intervention period. The estimated ``synthetic control'' can then help estimate the {\em future} (post-intervention) ground-truth measurements for all metrics associated with the treatment unit. 

\medskip
\noindent {\bf Algorithm and analysis.} The synthetic control literature \cite{abadie1, abadie2, abadie3, rsc1} relied on making the following 
key assumption: the treatment unit's measurements across time for the metric of interest can be expressed as a linear combination of the donor units' measurements. In this work, we start by arguing that we need not make this assumption as it holds naturally under the low-rank 3-order tensor model.  Furthermore, the low-rank 3-order tensor model suggests that the identical linear relationship holds across all metrics simultaneously. That is, in order to utilize measurements from other metrics to estimate the synthetic control for a given metric and a given unit of interest, in effect we can treat the measurements for other metric as additional measurements for our metric of interest! That is, in effect the number of pre-intervention measurements get multiplied by the number of available metrics. The resulting algorithm is natural adaption of the RSC algorithm but with multiple measurements, which we call the multidimensional robust synthetic control (mRSC). Using a recently developed method for analyzing error-in-variable regression in high-dimensional setup, we derive finite-sample guarantees on the performance of the mRSC algorithm. We conclude that the  pre- and post-intervention mean-squared-error (MSE) for mRSC decays faster than that of RSC by factor $K$ and $\sqrt{K}$ respectively, where $K$ is the number of metrics available. This formalizes the intuition that the data from other metrics effectively act as if the data belongs to the same metric. In summary, mRSC provides a way to overcome limited pre-intervention data by simply utilizing pre-intervention data across other metrics.

\medskip
\noindent {\bf Experiments: Synthetic data.} To begin with, we utilize synthetically generated data per our factor model to both verify tightness of theoretical results as well as understand the diagnostic test to determine whether the mRSC is applicable (or not). To begin with, we argue that if indeed mRSC is to work successfully, when we flatten the 3-order tensor of measurement data to a matrix by stacking the units by time slices across different metrics, the resulting matrix should have similar (approximate) rank as the matrix with only the single metric of interest (see Section \ref{sec:falsifiability} for details). We show that when the data is generated per our model, such test ought to be passed. And when data is not from our model, the test is failed. Next, we observe that the mRSC performs as predicted by theoretical results using experimental data. 

\medskip
\noindent {\bf Experiments: Retail.} Next, we study the efficacy of mRSC in a real-world dataset about departmental sales of product of Walmart obtained from Kaggle \cite{kaggle-walmart}. It comprises sales data for several product-departments across 45 store locations and 143 weeks. The store locations are units, weeks represent time and product-department represent different metric. Our goal is to forecast the sales of a given product-department at a given location after observing data for it pre-intervention, using data for all product-departments across all locations using both pre- and post-intervention data. We study the performance of mRSC and compare it with the RSC method across different intervention times and across different department-products as metric of choice. Across all our experiments, we consistently find that when pre-intervention data is very little, the mRSC method performs significantly better than RSC method; however, when there is a lot of pre-intervention data for a given metric of interest, then mRSC and RSC perform comparably. This is the behavior that is consistently observed and in line with our theoretical results: if pre-intervention data is very limited than the use of data from multiple metrics using mRSC provides significant gains. \todo[fancyline]{Dennis: any precise stats to be included here?}

\medskip
\noindent {\bf Experiments: Cricket.} We consider the task of forecasting trajectory in the game of cricket. 
This is an ideal candidate for mRSC because the game has {\em two} metrics of interest: runs scored and wickets lost. We provide
brief introduction to Cricket as we do not expect reader(s) to be familiar with the game, followed by why forecasting trajectory is
a perfect fit for mRSC setup and then summary of our findings. 

\smallskip
\noindent {\em Cricket 101.} Cricket, per Google Search for ``how many fans world-wide" seem to be the second most popular 
after soccer in the world at the time of this manuscript being written. It is played between two teams; it has inherently asymmetry 
in that both teams take turns to bat and bowl. While there are multiple formats with varying duration of the game, we focus on 
what is called ``50 overs Limited Over International (LOI)" format: each team bats for an ``inning" of 50 overs or 300 balls; during 
which at any given time two of its players (batsmen) are batting trying to score runs; while the other team fields all of its 11 players; 
one of which is bowling and others are fielding; collectively trying to get batsmen out or prevent them from scoring; and each 
batsman can get out at most once;  an inning ends when either 300 balls are done or 10 batsmen get out; at the end, team 
that makes more runs wins. 



%
%
%
%
%
%It is n asymmetric game 
%where both teams take turns to bat and bowl;
%
%is one of the most popular sports in the world. According to the BBC, over a billion people tuned in on television 
%to watch India play Pakistan in the ICC Cricket World Cup 2015 (\cite{bbccricket, wapocricket}). It is a fundamentally different 
%game compared to other popular sports: unlike football (soccer), rugby and basketball, cricket is an asymmetric game 
%where both teams take turns to bat and bowl; and unlike baseball, cricket has far fewer innings but each innings spans a 
%significantly longer amount of time. While cricket is played across three formats: the focus of this work is on the 50-over 
%Limited Overs International (LOI) games where each team only bats once and the winning team is the one that scores more 
%total runs. 
%
%A batting innings in a LOI cricket game is defined by the total number of times 
%the ball is bowled to a batter (similar to a ``pitch'' in baseball). In a 50-over LOI innings, the maximum number of balls bowled is $300$. 
%A group of six balls is called an ``over''. Therefore, for the format under consideration an innings can last up to $50$ overs or $300$ balls. 
%Each batting team gets a budget of $10$ ``outs'' which are defined as the number of times the team loses a batter. In cricket, a batter 
%getting ``out'' is also referred to as the team having lost a ``wicket''. Therefore, the state of a cricket innings is defined by the tuple of 
%({\em run scores}, {\em wickets lost}) at each point in the innings. We shall call the trajectory of an inning by sequence of such tuples
%at each of 300 balls. In the event that the team loses all $10$ of its wickets before the maximum number of balls (300) are bowled, 
%the innings ends immediately. The team batting second has to score one more runs than the team batting first to win the game. 
%As an example, in the ICC Cricket World Cup Final in 2015, New Zealand batted first and lost all ten wickets for a cumulative score of $183$ in 
%45 overs (270 balls). Australia were set a target of 184 in a maximum of 50 overs but they chased it successfully in 33 overs and 1 ball (199 balls) 
%for the loss of only 3 wickets.
%
%It is worth emphasizing that individuals comprising a team cannot change between innings. Everyone on the team can get to bat but 
%only a few typically bowl. The consequence of this is that a team typically comprises several specialists: some playing primarily as batters, 
%some primarily as bowlers with a few who are called upon to do both. Normally teams send their specialist batters to bat ahead of the bowling 
%specialists. This implies that the batting strength of a team degrades non-linearly, i.e. a loss of five wickets implies much more than 50\% of the 
%batting strength exhausted.

\smallskip
\noindent{\em Forecasting trajectory using mRSC.} As an important contribution, we utilize the mRSC algorithm for forecasting entire trajectory of the game using observation of initial parts of game. As a reader will notice, the utilization of mRSC for forecasting trajectory of game is generic and likely to be applicable to other games such as Basketball, which would be interesting future direction. To that end, we start by describing how mRSC can be utilized for forecasting trajectory of an ``inning''. We view each inning as a unit, the balls as time and score, wicket as two different metrics of interest. The historical innings are effectively donor units. The unit or inning of interest, for which we might have observed scores / wickets up to some number of initial balls (or time), is the treatment unit and the act of forecasting is simply coming up with ``synthetic control'' for this unit to estimate the score / wicket trajectory for future balls using it. And that's it. 

We collected data for historical LOI over the period of 1999-2017 for over 4700 innings. Each inning can be up to 300 balls long with score and wicket trajectory. We find that the approximately low-rank structure of matrix with only scores (4700 by 300) and that with both scores and wicket (4700 by 600) remains the same (see Figure \ref{fig:singvals}). This suggests that mRSC can be applicable for this scenario. 

%
%
%
%
%\medskip
%\noindent{\bf An mRSC Problem.} While it is not obvious a-priori, we show how the problem of forecasting scores trajectories in a cricket innings can be viewed as an instance of a multi-dimensional robust synthetic control problem. We show that the problem is a natural contender for the mRSC algorithm because there are two metrics of interest, i.e. runs scored and wickets lost, which are both essential to summarizing the state of the game. In the spirit of the mRSC model we introduce in this work, we model the runs scored and wickets lost on a given ball as random variables whose mean is a well-behaved, but arbitrary
%{\em latent} function of the {\em latent team context} parameter and {\em latent match condition} parameter. For example,
%team context parameter may include the team player condition, their current mental and physical state, effect of the ground on
%their performance, etc that primarily remain constant during the course of their innings. The match conditions parameter
%changes with every ball of the game and may capture aspects such as bowler, power play, weather, etc. 
%
%Every reasonable modeling assumption ought to be falsifiable and actual observations should not falsify the model. In
%that spirit, our model suggests that if we consider the matrices of score and wickets trajectories across all games played, where
%rows corresponds to different innings ever played, (up to 300) columns correspond to balls of the innings, and the value in
%the matrices correspond to the runs scored and wickets lost, then it must be {\em approximately} low rank. Putting it other way, their spectrum
%must decay quickly. Using historical data, we indeed find such as the case, see Figure \ref{fig:singvals}. Also note that a key feature of our model is that the matrices of runs, wickets and their combination (via concatenation) appear to retain a similar rank which serves as a validation of the mRSC model discussed in Section \ref{sec:model}.


%\noindent{\bf Parsimonious model.} We propose a parsimonious generative model for the runs scored and wickets lost trajectories in cricket. Amongst cricketing pundits and fans, it is 
%generally believed that the performance of a team's innings depends on the team under consideration, playing
%conditions and the match situation. In a sense, this is a generic philosophy applies to most sports. To formalize
%this, we model the runs scored and wickets lost on a given ball as random variables whose mean is a well-behaved, but arbitrary
%{\em latent} function of the {\em latent team context} parameter and {\em latent match condition} parameter. For example,
%team context parameter may include the team player condition, their current mental and physical state, effect of the ground on
%their performance, etc that primarily remain constant during the course of their innings. The match conditions parameter
%changes with every ball of the game and may capture aspects such as bowler, power play, weather, etc. We 
%model the {\em well behaved} aspect of the latent function through Lipschitz continuity, but the choice of function arbitrary otherwise. We note
%that the latent parameter need not be one-dimensional, and is likely higher dimensional. 


%\smallskip
%\noindent{\bf Forecasting.} The approximately low-rank structure of the combined runs and wickets trajectory matrix naturally leads to the mRSC algorithm introduced earlier. We introduce arbitrary interventions, e.g. at the 30th over (180 balls), use the pre-intervention data matrix to estimate the synthetic control weights and then use them to estimate the future trajectories (for runs and wickets) for the innings of interest.

%Specifically,
%consider the innings that is ongoing and we wish to forecast the remainder of its trajectory. In effect, we can
%view this innings as one of the rows in the trajectories matrix. The trajectories matrix is approximately
%low rank, which means that if we took a random row from this matrix, it is likely to be an approximately linear combination
%of {\em few} other rows in the matrix. Therefore, it is reasonable to hypothesize that the incomplete row of interest can also be
%expressed as linear combination of few of the complete rows of the trajectories matrix. And this linear combination can
%be found by solving an appropriate linear regression using the observed part of the incomplete trajectory. Then, we 
%can extrapolate or forecast the score trajectory of interest by simply taking the linear combination estimated using complete trajectories. 
%In effect, this is precisely what a synthetic control procedure does \cite{abadie1, abadie2}. In the robust version,
%as the first step, data is de-noised by applying matrix estimation on the score trajectory matrix to remove the noise \cite{rsc1}. 

Next, we evaluate the performance on more than 750 recent (2010 to 2017) LOI innings. For consistency of comparisons, 
we conduct detailed study  for forecasting at the 30 overs or 180 balls (i.e. 60\% of the inning).  We measure performance 
through Mean-Absolute-Percentage-Error (MAPE) and R-square (R2). The median of the MAPE of our forecasts varies 
from $0.027$ or $2.7$\% for 5 overs ahead to $0.051$ or $5.1$\% for 20 overs ahead. While this, on its own is significant, 
to get a sense of the {\em absolute} performance, we evaluate the $R^2$ of our forecasts. We find that the $R^2$ of 
our forecast varies from $0.92$ for 5 overs to $0.79$ for 15 overs. That is, for 5 over forecasting, we can explain $92$\% of 
``variance'' in the data, which is surprisingly accurate. Finally, we establish the value of the the de-noising and regression steps 
in the mRSC algorithm. Through one important experiment we also establish that the commonly held belief that the donor 
pool should only comprise innings involving the same team for which we are interested in forecasting leads to worse estimation. 
This is related to {\em Stein's Paradox} \cite{stein1} which was observed in baseball. Finally, we show using examples of actual 
cricket games that the mRSC algorithm successfully captures and reacts to nuances of the game of cricket. 

\subsection{Organization} The rest of this work is organized as follows: we review the relevant bodies of literature next (Section \ref{sec:related} followed by a
detailed overview of the problem and our proposed model (Section \ref{sec:model}). Next, in Section \ref{sec:algorithm} we describe the setting and the mRSC algorithm which is followed by a simple
diagnostic test to determine model applicability to a problem. We present the main theoretical results in Section \ref{sec:results} followed by a synthetic experiment and ``real-world'' retail case study to
compare the mRSC algorithm to the RSC (Section \ref{sec:experiments}). Finally, in Section \ref{sec:cricket} we have the complete case study for the game of cricket to demonstrate the versatility of the proposed
model and superior predictive performance.
%
%Naturally, we do not include
%the innings for which we wish to forecast as part of our donor pool. While forecasting can be done at any point along the trajectory,
%to be able to compare across various settings, we conduct a detailed study for forecasting at the 30 overs or 180 balls (i.e. 60\% of the inning).  
%To evaluate the forecasting performance, we compute the error for each future ball of the trajectory with respect to the
%ground truth. We use the Mean-Absolute-Percentage-Error (MAPE) and R-square (R2) to evaluate the forecast quality. 

%The median of the MAPE of our forecasts varies from $0.027$ or $2.7$\% for 5 overs ahead to $0.051$ or $5.1$\% for 20 overs ahead. 
%While this, on its own is significant, to get a sense of the {\em absolute} performance, we evaluate the $R^2$ of our forecasts. We
%find that the $R^2$ of our forecast varies from $0.92$ for 5 overs to $0.79$ for 15 overs. That is, for 5 over forecasting, we can explain
%$92$\% of ``variance'' in the data, which is surprisingly accurate. 

%We also establish the value of the the de-noising and regression steps in the mRSC algorithm. Through one important experiment we also establish that the commonly held belief that the donor pool should only comprise innings involving the same team for which we are interested in forecasting leads to worse estimation. This is related to {\em Stein's Paradox} \cite{stein1} which was observed in baseball. Finally, we show using examples of actual cricket games that the mRSC algorithm successfully captures and reacts to nuances of the game of cricket. 


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../cricket"
%%% End:


==> content/introduction_ds.tex <==
\section{Introduction} \label{sec:intro}

Quantifying the causal statistical effect of interventions is a problem of interest across a wide array of domains. 
From policy making to engineering and medicine, estimating the effect of an intervention is critical for innovation and understanding 
existing systems. In any setting, with or without an intervention, we only observe one set of outcomes. In casual 
analysis, the fundamental problem is that of estimating what wasn't observed, i.e., the {\em counterfactual}. 
%
%
% i.e. another set of outcomes. Specifically, when evaluating the effect of a treatment on a unit of interest, we observe the effects of that treatment. In order to quantify the effect as significant (or not), the counterfactual must be estimated, i.e. the unobserved outcomes that {\em would have} happened {\em without} the intervention. Our focus is on this problem of estimating the counterfactual. 
% 
% Specifically, given an arbitrary intervention point, our problem of interest is to estimate what would have happened if there was no {\em actual} intervention and things continued in the same vein as before the arbitrarily chosen evaluation point.

We consider the setting of observational studies where experimental studies are not feasible to estimate the {\em counterfactual}. In order to estimate the counterfactual, observational studies rely on the identification (or estimation) of a {\em control} unit. This can be achieved by relying on expert domain knowledge, or via techniques such as {\em matching} the target unit to existing control units (called {\em donors}) on covariates features or propensity scores. A popular data-driven approach to estimating the control unit is known as the synthetic control (SC) method  \cite{abadie1, abadie2, abadie3}. SC assigns convex weights to the donors such that the resulting {\em synthetic} unit most closely matches the target unit according to a chosen metric of interest. A generalization of this approach, known as robust synthetic control (RSC) \cite{rsc1}, removes the convexity constraint and guarantees a consistent estimator that is robust to missing data and noise. 

While SC, its many variants, and RSC exhibit attractive properties, they all suffer for poor estimation when 
the amount of training data (i.e., the length of the pre-intervention period) is small. 

In many scenarios with little pre-intervention data, there is, however, data available for many different types which might be related to the type of data of interest. For example, we might be interested in crime-rate 
and there might be related data available such as median income of house-hold, graduation rate from high-school. Therefore, one remedy to 
the limited pre-intervention data is to utilize data from multiple metrics. 
As the main contribution of this work, we address this challenge by providing 

%
%\subsection{Problem Statement}
%Given a unit of interest say unit $1$, $N-1$ donor units and data for $K > 1$ metrics observed for $T_0$ time periods (for all $N$ units), 
%the problem considered in this work is that of estimating the mean {\em synthetic} control unit for the unit of interest. 
%
%Additionally, it is our goal to use the synthetic control to estimate, or {\em forecast}, the mean counterfactual for the unit of interest (for all $K$ metrics) from time periods $(T_0, T]$.
%
%%\todo[inline]{We need to clarify here that our interest in this paper is not the counterfactual for analyzing impact of an actual intervention, rather it is for timeseries prediction}
%
%Here we note that for most of the experimentation in this work we use arbitrary {\em interventions} which should have no statistical effect. Our goal is to use the observed data to estimate the mean effects {\em without} any changes. Therefore, we are only concerned with the problems of estimation of the control unit and its forecasts (counterfactual). 

\subsection{Contributions}

As the main contribution of this work, we address this challenge of poor estimation of counterfactual \todo[inline]{Do we want the main contribution to address the poor estimation issue? Isn't the generalization of RSC to mRSC important without the poor estimation issue?} due to limited pre-intervention data by providing a generalization of RSC method, the mRSC, which incorporates multiple-types of data in a principled manner. We show that our mRSC method is a natural consequence of the popular factor model. Through this connection, we provide a falsifiability test for mRSC in a data-driven manner. In particular, we establish that if test is passed, then mRSC produces a consistent estimation of the mean unit of interest (for all metrics) in the pre- and post-intervention periods. Further, the accuracy of estimating control using mRSC improves with respect to the RSC with increasing number of different types of relevant data. Specifically, the Mean Squared Error (MSE) is decreased by a factor of $K$ and $\sqrt{K}$ for the pre- and post-intervention estimates. All other properties of the RSC algorithm, namely robustness to missing data and noise, all carry over. Finally, we conduct extensive experimentation to establish the efficacy of this generalized method in comparison to the RSC algorithm via synthetically generated 
datasets and two real-world case-studies: product sales in retail and trajectory forecasting in game of Cricket. Next, we summarize these contributions in more detail.

\medskip
\noindent {\bf Model.} We consider a natural generalization of the factor (or latent variable) model considered in the literature cf. \cite{rsc1} where the measurement associated with a unit, at a given time for a given metric is function of features associated with unit, time and the metric. A special case of such models, the linear factor models, are "bread and butter" model within the Econometrics literature and assumed in \cite{abadie1, abadie2, abadie3}. We argue that  as long as function is Lipschitz and features belong to compact domain, the resulting factor model can be well approximated by low-rank 3-order tensor with three dimensions of tensor corresponding to unit, time and metric respectively. Therefore, for simplicity of exposition, we focus on setup where the underlying model is indeed a low-rank 3-order tensor. The observations are noisy version of the ground truth 3-order low-rank tensor with potentially missing values. These include pre-intervention data for all units and metrics, while post-intervention data only for ``donor'' units. The goal is to learn the ``synthetic control'' across donor units and all the metrics simultaneously using pre-intervention data so that using post-intervention data for donor units and metrics, the learnt ``synthetic control'' can help estimate the ground-truth measurements for all metrics associated with the treatment unit post-intervention. 

\medskip
\noindent {\bf Algorithm and analysis.} The synthetic control literature \cite{abadie1, abadie2, abadie3, rsc1} relied on making the following 
key assumption: the treatment unit's measurements across time for the metric of interest can be expressed as a linear combination of the donor units' measurements. In this work, we start by arguing that we need not make this assumption as it holds naturally under the low-rank 3-order tensor model.  Furthermore, the low-rank 3-order tensor model suggests that the identical linear relationship holds across all metrics simultaneously. That is, in order to utilize measurements from other metrics to learn synthetic control for a given metric and a given unit of interest, in effect we can treat the measurements for other metric as additional measurements for our metric of interest! That is, in effect the measurements pre-intervention get multiplied by the number of available metrics. The resulting algorithm is natural adaption of the RSC algorithm but with multiple measurements, which we call the multi-dimensional robust synthetic control (mRSC). Using a recently developed method for analyzing error-in-variable regression in high-dimensional setup, we derive finite-sample guarantees on the performance of our mRSC algorithm. We conclude that the mean-squared-error (MSE) for mRSC pre- and post-intervention decays faster than that of RSC by factor $K$ and $\sqrt{K}$ respectively, where $K$ is the number of metrics available. This formalizes the intuition that the data from other metric effectively act as if the data from the same metric. In summary, mRSC provides a way to overcome limited pre-intervention data by simply utilizing pre-intervention data across many metrics.

\medskip
\noindent {\bf Experiments: Synthetic data.} To begin with, we utilize synthetically generated data per our factor model to both verify tightness of theoretical results as well as understand the diagnostic test to see when is mRSC applicable (or not). To begin with, we argue that if indeed mRSC is to work successfully, when we flatten the 3-order tensor of measurement data to matrix by stacking the unit by time slices across different metric side-by-side (see Section \ref{sec:falsifiability} for details), the result matrix should have similar (approximate) rank as the matrix with only the single metric of interest. We show that when the data is per our model, such test ought to be passed. And when data is not from our model, the test is failed. Next, we observe that the mRSC performs as predicted by theoretical results using experimental data. 

\medskip
\noindent {\bf Experiments: Retail.} Next, we study the efficacy of mRSC in a real-world dataset about departmental sales of product of Walmart obtained from Kaggle \cite{kaggle-walmart}. It comprises sales data for several product-departments across 45 store locations and 143 weeks. The store locations are units, weeks represent time and product-department represent different metric. Our goal is to forecast the sales of a given product-department at a given location after observing data for it pre-intervention, using data for all product-departments across all locations using both pre- and post-intervention data. We study the performance of mRSC and compare it with the RSC method across different intervention times and across different department-products as metric of choice. Across all our experiments, we consistently find that when pre-intervention data is very little, the mRSC method performs significantly better than RSC method; however, when there is a lot of pre-intervention data for a given metric of interest, then mRSC and RSC perform comparably. This is the behavior that is consistently observed and in line with our theoretical results: if pre-intervention data is very limited than the use of data from multiple metrics using mRSC provides significant gains. \todo[fancyline]{Dennis: any precise stats to be included here?}

\medskip
\noindent {\bf Experiments: Cricket.} We consider the task of forecasting trajectory in the game of cricket. 
This is an ideal candidate for mRSC because the game has {\em two} metrics of interest: runs scored and wickets lost. We provide
brief introduction to Cricket as we do not expect reader(s) to be familiar with the game, followed by why forecasting trajectory is
a perfect fit for mRSC setup and then summary of our findings. 

\smallskip
\noindent {\em Cricket 101.} Cricket, per Google Search for ``how many fans world-wide" seem to be the second most popular 
after soccer in the world at the time of this manuscript being written. It is played between two teams; it has inherently asymmetry 
in that both teams take turns to bat and bowl. While there are multiple formats with varying duration of the game, we focus on 
what is called ``50 overs Limited Over International (LOI)" format: each team bats for an ``inning" of 50 overs or 300 balls; during 
which at any given time two of its players (batsmen) are batting trying to score runs; while the other team fields all of its 11 players; 
one of which is bowling and others are fielding; collectively trying to get batsmen out or prevent them from scoring; and each 
batsman can get out at most once;  an inning ends when either 300 balls are done or 10 batsmen get out; at the end, team 
that makes more runs wins. 



%
%
%
%
%
%It is n asymmetric game 
%where both teams take turns to bat and bowl;
%
%is one of the most popular sports in the world. According to the BBC, over a billion people tuned in on television 
%to watch India play Pakistan in the ICC Cricket World Cup 2015 (\cite{bbccricket, wapocricket}). It is a fundamentally different 
%game compared to other popular sports: unlike football (soccer), rugby and basketball, cricket is an asymmetric game 
%where both teams take turns to bat and bowl; and unlike baseball, cricket has far fewer innings but each innings spans a 
%significantly longer amount of time. While cricket is played across three formats: the focus of this work is on the 50-over 
%Limited Overs International (LOI) games where each team only bats once and the winning team is the one that scores more 
%total runs. 
%
%A batting innings in a LOI cricket game is defined by the total number of times 
%the ball is bowled to a batter (similar to a ``pitch'' in baseball). In a 50-over LOI innings, the maximum number of balls bowled is $300$. 
%A group of six balls is called an ``over''. Therefore, for the format under consideration an innings can last up to $50$ overs or $300$ balls. 
%Each batting team gets a budget of $10$ ``outs'' which are defined as the number of times the team loses a batter. In cricket, a batter 
%getting ``out'' is also referred to as the team having lost a ``wicket''. Therefore, the state of a cricket innings is defined by the tuple of 
%({\em run scores}, {\em wickets lost}) at each point in the innings. We shall call the trajectory of an inning by sequence of such tuples
%at each of 300 balls. In the event that the team loses all $10$ of its wickets before the maximum number of balls (300) are bowled, 
%the innings ends immediately. The team batting second has to score one more runs than the team batting first to win the game. 
%As an example, in the ICC Cricket World Cup Final in 2015, New Zealand batted first and lost all ten wickets for a cumulative score of $183$ in 
%45 overs (270 balls). Australia were set a target of 184 in a maximum of 50 overs but they chased it successfully in 33 overs and 1 ball (199 balls) 
%for the loss of only 3 wickets.
%
%It is worth emphasizing that individuals comprising a team cannot change between innings. Everyone on the team can get to bat but 
%only a few typically bowl. The consequence of this is that a team typically comprises several specialists: some playing primarily as batters, 
%some primarily as bowlers with a few who are called upon to do both. Normally teams send their specialist batters to bat ahead of the bowling 
%specialists. This implies that the batting strength of a team degrades non-linearly, i.e. a loss of five wickets implies much more than 50\% of the 
%batting strength exhausted.

\smallskip
\noindent{\em Forecasting trajectory using mRSC.} As an important contribution, we utilize the mRSC algorithm for forecasting entire trajectory of the game using observation of initial parts of game. As a reader will notice, the utilization of mRSC for forecasting trajectory of game is generic and likely to be applicable to other games such as Basketball, which would be interesting future direction. To that end, we start by describing how mRSC can be utilized for forecasting trajectory of an ``inning''. We view each inning as a unit, the balls as time and score, wicket as two different metrics of interest. The historical innings are effectively donor units. The unit or inning of interest, for which we might have observed scores / wickets up to some number of initial balls (or time), is the treatment unit and the act of forecasting is simply coming up with ``synthetic control'' for this unit to estimate the score / wicket trajectory for future balls using it. And that's it. 

We collected data for historical LOI over the period of 1999-2017 for over 4700 innings. Each inning can be up to 300 balls long with score and wicket trajectory. We find that the approximately low-rank structure of matrix with only scores (4700 by 300) and that with both scores and wicket (4700 by 600) remains the same (see Figure \ref{fig:singvals}). This suggests that mRSC can be applicable for this scenario. 

%
%
%
%
%\medskip
%\noindent{\bf An mRSC Problem.} While it is not obvious a-priori, we show how the problem of forecasting scores trajectories in a cricket innings can be viewed as an instance of a multi-dimensional robust synthetic control problem. We show that the problem is a natural contender for the mRSC algorithm because there are two metrics of interest, i.e. runs scored and wickets lost, which are both essential to summarizing the state of the game. In the spirit of the mRSC model we introduce in this work, we model the runs scored and wickets lost on a given ball as random variables whose mean is a well-behaved, but arbitrary
%{\em latent} function of the {\em latent team context} parameter and {\em latent match condition} parameter. For example,
%team context parameter may include the team player condition, their current mental and physical state, effect of the ground on
%their performance, etc that primarily remain constant during the course of their innings. The match conditions parameter
%changes with every ball of the game and may capture aspects such as bowler, power play, weather, etc. 
%
%Every reasonable modeling assumption ought to be falsifiable and actual observations should not falsify the model. In
%that spirit, our model suggests that if we consider the matrices of score and wickets trajectories across all games played, where
%rows corresponds to different innings ever played, (up to 300) columns correspond to balls of the innings, and the value in
%the matrices correspond to the runs scored and wickets lost, then it must be {\em approximately} low rank. Putting it other way, their spectrum
%must decay quickly. Using historical data, we indeed find such as the case, see Figure \ref{fig:singvals}. Also note that a key feature of our model is that the matrices of runs, wickets and their combination (via concatenation) appear to retain a similar rank which serves as a validation of the mRSC model discussed in Section \ref{sec:model}.


%\noindent{\bf Parsimonious model.} We propose a parsimonious generative model for the runs scored and wickets lost trajectories in cricket. Amongst cricketing pundits and fans, it is 
%generally believed that the performance of a team's innings depends on the team under consideration, playing
%conditions and the match situation. In a sense, this is a generic philosophy applies to most sports. To formalize
%this, we model the runs scored and wickets lost on a given ball as random variables whose mean is a well-behaved, but arbitrary
%{\em latent} function of the {\em latent team context} parameter and {\em latent match condition} parameter. For example,
%team context parameter may include the team player condition, their current mental and physical state, effect of the ground on
%their performance, etc that primarily remain constant during the course of their innings. The match conditions parameter
%changes with every ball of the game and may capture aspects such as bowler, power play, weather, etc. We 
%model the {\em well behaved} aspect of the latent function through Lipschitz continuity, but the choice of function arbitrary otherwise. We note
%that the latent parameter need not be one-dimensional, and is likely higher dimensional. 


%\smallskip
%\noindent{\bf Forecasting.} The approximately low-rank structure of the combined runs and wickets trajectory matrix naturally leads to the mRSC algorithm introduced earlier. We introduce arbitrary interventions, e.g. at the 30th over (180 balls), use the pre-intervention data matrix to estimate the synthetic control weights and then use them to estimate the future trajectories (for runs and wickets) for the innings of interest.

%Specifically,
%consider the innings that is ongoing and we wish to forecast the remainder of its trajectory. In effect, we can
%view this innings as one of the rows in the trajectories matrix. The trajectories matrix is approximately
%low rank, which means that if we took a random row from this matrix, it is likely to be an approximately linear combination
%of {\em few} other rows in the matrix. Therefore, it is reasonable to hypothesize that the incomplete row of interest can also be
%expressed as linear combination of few of the complete rows of the trajectories matrix. And this linear combination can
%be found by solving an appropriate linear regression using the observed part of the incomplete trajectory. Then, we 
%can extrapolate or forecast the score trajectory of interest by simply taking the linear combination estimated using complete trajectories. 
%In effect, this is precisely what a synthetic control procedure does \cite{abadie1, abadie2}. In the robust version,
%as the first step, data is de-noised by applying matrix estimation on the score trajectory matrix to remove the noise \cite{rsc1}. 

Next, we evaluate the performance on more than 750 recent (2010 to 2017) LOI innings. For consistency of comparisons, 
we conduct detailed study  for forecasting at the 30 overs or 180 balls (i.e. 60\% of the inning).  We measure performance 
through Mean-Absolute-Percentage-Error (MAPE) and R-square (R2). The median of the MAPE of our forecasts varies 
from $0.027$ or $2.7$\% for 5 overs ahead to $0.051$ or $5.1$\% for 20 overs ahead. While this, on its own is significant, 
to get a sense of the {\em absolute} performance, we evaluate the $R^2$ of our forecasts. We find that the $R^2$ of 
our forecast varies from $0.92$ for 5 overs to $0.79$ for 15 overs. That is, for 5 over forecasting, we can explain $92$\% of 
``variance'' in the data, which is surprisingly accurate. Finally, we establish the value of the the de-noising and regression steps 
in the mRSC algorithm. Through one important experiment we also establish that the commonly held belief that the donor 
pool should only comprise innings involving the same team for which we are interested in forecasting leads to worse estimation. 
This is related to {\em Stein's Paradox} \cite{stein1} which was observed in baseball. Finally, we show using examples of actual 
cricket games that the mRSC algorithm successfully captures and reacts to nuances of the game of cricket. 

\subsection{Organization} The rest of this work is organized as follows: we review the relevant bodies of literature (Section \ref{sec:related}) followed by a
detailed overview of the problem and our proposed model (Section \ref{sec:model}). Next, in Section \ref{sec:algorithm}, we describe the setting and the mRSC algorithm. We present the main theoretical results in Section \ref{sec:results} followed by a synthetic experiment and ``real-world'' retail case study to
compare the mRSC algorithm to the RSC (Section \ref{sec:experiments}) in the presence of sparse data. Finally, in Section \ref{sec:cricket}, we have the complete case study for the game of cricket to demonstrate the versatility of the proposed
model and its superior predictive performance.

% with details  is followed by a simple diagnostic test to determine model applicability to a problem

%
%Naturally, we do not include
%the innings for which we wish to forecast as part of our donor pool. While forecasting can be done at any point along the trajectory,
%to be able to compare across various settings, we conduct a detailed study for forecasting at the 30 overs or 180 balls (i.e. 60\% of the inning).  
%To evaluate the forecasting performance, we compute the error for each future ball of the trajectory with respect to the
%ground truth. We use the Mean-Absolute-Percentage-Error (MAPE) and R-square (R2) to evaluate the forecast quality. 

%The median of the MAPE of our forecasts varies from $0.027$ or $2.7$\% for 5 overs ahead to $0.051$ or $5.1$\% for 20 overs ahead. 
%While this, on its own is significant, to get a sense of the {\em absolute} performance, we evaluate the $R^2$ of our forecasts. We
%find that the $R^2$ of our forecast varies from $0.92$ for 5 overs to $0.79$ for 15 overs. That is, for 5 over forecasting, we can explain
%$92$\% of ``variance'' in the data, which is surprisingly accurate. 

%We also establish the value of the the de-noising and regression steps in the mRSC algorithm. Through one important experiment we also establish that the commonly held belief that the donor pool should only comprise innings involving the same team for which we are interested in forecasting leads to worse estimation. This is related to {\em Stein's Paradox} \cite{stein1} which was observed in baseball. Finally, we show using examples of actual cricket games that the mRSC algorithm successfully captures and reacts to nuances of the game of cricket. 


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../cricket"
%%% End:


==> content/main_results.tex <==
\section{Main Results} \label{sec:results}

We now present our main results, which bound the pre- and post-intervention prediction errors of our algorithm. 



==> content/model.tex <==
\section{Model} \label{sec:cricketmodel}

\smallskip
\noindent{\bf Intuition.} 
We shall introduce the {\em Latent Variable Model} here. It is motivated by the following minimal property 
that sports fans and pundits expect to hold for variety of sports: performance of a team is determined by
the {\em team context} that remains constant during the duration of the game and the {\em game context}
that changes during the play of the game. In cricket, {\em team context} may correspond to players in the team, 
coach, the mental state in which the players are, the importance of the game (e.g. final of the world cup), 
the venue of game and fan base, the pitch or ground condition, etc. And, the {\em game context} may 
correspond to stage of the game, power play, etc. Next, we formalize this seemingly universal intuition
across sports in the context of cricket. 

\smallskip
\noindent{\bf Formalism.} 
The performance, as mentioned before, is measured by the runs scored and the wickets lost. To that
end, we shall index an inning by $i$, and ball within the inning by $j$. Let there be total of $n$ innings
and $b$ balls, within LOI, $b = 300$. Let $X_{ij}$ denote the runs on the ball $j$ within inning $i$. 
We shall model $X_{ij}$ as independent random variables with mean $m_{ij} = {\mathbb E}[X_{ij}]$. 
To capture the above stated intuition, we state that 
\begin{align}
m_{ij} & = f(\theta_i, \rho_j), 
\end{align}
for all $i \in [n], j \in [b]$\footnote{We use notation $[x] = \{1,\dots, x\}$ for integer $x$.} where 
{\em latent} parameter $\theta_i \in \Omega_1 = [r_1, s_1]^{d_1}$ captures the {\em team context},
{\em latent} parameter $\rho_j \in \Omega_2 = [r_2, s_2]^{d_2}$ captures the {\em game context}, 
and {\em latent} function $f: \Omega_1 \times \Omega_2 \to [0,\infty)$ captures complexity of the
underlying model. For simplicity and without loss of generality, we shall assume that $r_1=r_2 = 0$,
$s_1 = s_2 = 1$, $d_1 = d_2 = d \geq 1$. 

We shall additionally impose that the latent function $f$ is {\em Lipschitz} continuous, but can be 
arbitrary otherwise. That is, there exists constant $C_f > 0$ such that for all $\theta, \theta' \in \Omega_1$
and $\rho, \rho' \in \Omega_2$, 
\begin{align}
|f(\theta, \rho) - f(\theta', \rho')| & \leq C_f \Big(\| \theta - \theta'\|  + \| \rho - \rho'\|\Big).
\end{align}
From the modeling perspective, restriction of Lipschitz continuity on $f$  is mild and states that performance
of a team can not change arbitrarily when team context and / or game context changes mildly, which makes 
sense. 

\smallskip
\noindent{\bf Implication.} 
Consider the matrix of runs scored across all $n$ innings and all $b$ balls, $\bX = [X_{ij}] \in {\mathbb N}^{n \times b}$. 
Therefore, ${\mathbb E}[\bX] = \bm = [m_{ij}] = [f(\theta_i, \rho_j)]$. Define $Y_{ij} = \sum_{k=1}^j X_{ik}$ as the cumulative 
runs scores in the inning $i$ up to and including $j$th ball and let $\bY = [Y_{ij}] \in {\mathbb N}^{n \times b}$. Then, 
${\mathbb E}[Y_{ij}] = \sum_{k=1}^j m_{ik}$. Also, let $\bM = {\mathbb E}[\bY]$. 

\begin{proposition}\label{prop:low-rank}
For any $\varepsilon > 0$, there exists $r = r(\varepsilon, d) \geq 1$ such that matrix $\bfm$ is approximated by a
matrix of rank $r(\varepsilon, d)$ with respect to entry-wise max-norm within $\varepsilon$. That is, there exists
matrix $\bfm^{(r)}$ of rank $r$ such that $\max_{i,j} |m_{ij} - m^{(r)}_{ij}| \leq \varepsilon$. Subsequently, matrix
$\bM^{(r)} = [M^{(r)}_{ij}]$ where $M^{(r)}_{ij} = \sum_{k=1}^j m^{(r)}_{ik}$ is of rank at most $r$ and approximates
$\bM$ such that $\max_{ij} | M_{ij} - M^{(r)}_{ij}| \leq b \varepsilon$. 
\end{proposition}
For the proof of Proposition, we refer the reader to the Appendix (Section \ref{sec:appendix_proof_prop}).\\
%\begin{proof} The proof is a straight forward extension of the arguments in \cite{usvt} and \cite{amjadshah1}. First, we consider the matrix $\bfm = [m_{ij}], \forall{i} \in [n], \forall{j} \in [b]$. Recall that $m_{ij} = f(\theta_i, \rho_j)$ where $f(\cdot)$ is Lipschitz in its arguments with the Lipschitz constant, $C_f > 0$. We have assumed that the latent parameters belong to a compact space: $[0, 1]^d$, where $d \geq 1$. Given that the number of columns are typically much smaller than the number of rows, i.e. $b << n$, we define a finite covering, $P(\eps)$, such that the following holds: for any $A \in P(\eps)$, whenever $\rho, \rho'$ are two points such that $\rho, \rho' \in A$ we have $| f(\theta_i, \rho) -  f(\theta_i, \rho') | \leq \eps$. Due to the Lipschitzness of the function $f$ and the compactness of any finite subinterval of $[0,1]^d$ it can be shown that $| P(\eps) | \leq C(C_f, d) \eps^{-d}$, where $C(C_f, d)$ is a constant which depends only on the Lipschitz constant, $C_f$, and the dimension of the latent space, $d$.  (see \cite{amjadshah1}).
%
%We now construct the matrix $\bfm^{(r)}$. For latent feature $\rho_j$ corresponding to the column $j \in [b]$, find closest element in $P(\eps)$ and let it be denoted by $p(\rho_j)$. Create the matrix $\bfm^{(r)} = [m_{ij}^{(r)}]$ where $m_{ij}^{(r)}= f(\theta_i, p(\rho_j))$. We note that $\text{rank}(\bfm^{(r)}) = r =  | P(\eps) | \leq C(C_f, d) \eps^{-d} = r(C_f, d, \eps)$. In the manner in which we have constructed $P(\eps)$ and $\bfm^{(r)}$, we know that $m_{ij} - m_{ij}^{(r)} \leq \eps$. Therefore, $\max_{i,j} |m_{ij} - m^{(r)}_{ij}| \leq \varepsilon$, as required.
%
%Next, we consider the cumulative column matrix, $\bM$. First consider that the number of distinct rows (or columns) in $\bfm$ is less than the rank $r = r(C_f, d, \eps)$. Note that each column, $j$, in $\bM$ is generated by taking a sum of all columns $k$, where $1 \leq k \leq j$. Therefore, the relationship between the rows of $\bfm$ is maintained in the rows of $\bM$. This implies that the $\text{rank}(\bM) \leq \text{rank}(\bfm) = r(C_f, d, \eps)$. Finally, given that the last column, $b$, in $\bM$ is the cumulative sum of all columns $k$ where $1 \leq k \leq b$, it must be that $\max_{i,j} |M_{ij} - M^{(r)}_{ij}| \leq b \max_{i,j} |m_{ij} - m^{(r)}_{ij}| = b\varepsilon$.
%\end{proof}
\smallskip
\noindent{\bf Falsifiability.} 
The Proposition \ref{prop:low-rank} suggests that if indeed our model assumption holds in practice, then the
data matrix of score trajectories, $\bY$ ought to be well approximated by low-rank. Putting it other way, its spectrum
out to be concentrated on top few principle components. This gives us way to test falsifiability of our model for the game
of cricket, and more generally any game of interest. 

In the context of cricket, we consider matrix comprising over 4700 LOI innings from 1999 to 2017, i.e. as many rows and $300$
columns. Figure \ref{fig:singvals} shows the spectrum of the top 15\% singular values (sorted in descending order) for this matrix. Note that the matrix has been normalized to re-scale all scores to remain between the range $[-1, 1]$. It clearly supports the implications that most of the spectrum is concentrated in the top $8$ principle components. Indeed, we note that the over 99.9\% of the ``energy'' in the matrix is captured by the top 8 singular values. We determine this by calculating the ratio of the sum of squares of the top 8 singular values to the sum of squares of all singular values of this matrix.

\smallskip
\noindent{\bf Implied linear relationship.} The approximately low-rank structure of the mean matrix $\bm$ and hence $\bM$ per
Proposition \ref{prop:low-rank} for Latent Variable Model and verified through data suggests that if we choose a row (or inning)
at random, then it is well approximated by a linear combination of {\em few} other rows. We formalize this implication by
making the following assumption. For a new cricket innings, the mean cumulative score performance $M \in \RealsP^b$ 
can be represented as a linear  combination of the mean score performance of other existing innings: 
\begin{align} \label{eq:assumption2}
M = \sum_{i=1}^{n} \beta_i M_i,
\end{align}
and $\beta_i \in \mathbb{R}$ are weights that depend on the inning of interest and $M_i = [M_{ij}]_{j \in [b]} \in \RealsP^b$. 

%
%
%We denote the maximum number of balls in an innings by $b$. As an example, in a Limited Overs International (LOI) game, we assume 50 overs ($b = 300$ balls). We view each batting innings as a sequence of 300 ordered observations. We have access to $n$ such innings across history. There are two key cricketing insights that will guide the appropriate modeling framework for cricket innings.
%
%\begin{itemize}
%\item \textbf{Key Insight 1}: there is {\em memory} in cricket innings. Anecdotally, fans of the game often comment that passages of play resemble instances from past games that they recall. If this is indeed true, a reasonable model must be successful at inferring and exploiting such relationships.
%
%\item \textbf{Key Insight 2}: the evolution of an innings is a complex function of the playing conditions, the teams under consideration and the match situation etc. This implies that any model that relies only on the current state (at the time of intervention) but ignores the history of the observations before the intervention, will be unable to exploit contextual information relevant to an innings. A reasonable model must take \textit{context} in to account.
%\end{itemize}
%
%These two key insights help us model a cricket innings using the Latent Variable Model (LVM) introduced as the unified modeling framework earlier in this work (Chapter \ref{chap:intro}). Formally, let $Y_{ij}$ represent a random variable which denotes the cumulative runs scored in innings $i$ up to and including ball $j$.  We propose the following model:
%\begin{align} \label{eq:model1}
%Y_{ij}  &= m_{ij} + \eps_{ij},
%\end{align}
%where $\eps_{ij}$ is zero-mean random noise which is independent across all innings, $1 \leq i \leq n$, and balls, $1 \leq j \leq b$. This implies
%\begin{align} \label{eq:model2}
%\mathbb{E}[Y_{ij}]  &= m_{ij}
%\end{align}
%
%Given that $\eps_{ij}$ is independent noise, the quantity of interest for our inference and forecasting problems is $m_{ij}$. We use the latent variable model (LVM) to assume that $m_{ij}$ is a function of some contextual row- and column- latent parameters $(\theta_i, \rho_j)$, i.e.:
%
%\begin{align} \label{eq:model4}
%\mathbb{E}[Y_{ij}] = m_{ij} &= \boldsymbol{f}(\theta_i, \rho_j),
%\end{align}
%where $\theta_i \in \Omega_1 = [r_1, s_1]^{d_1}$ and $\rho_j \in \Omega_2 = [r_2, s_2]^{d_2}$. $\Omega_1$ and $\Omega_2$ are compact spaces in $\mathbb{R}^{d_1}$ and $\mathbb{R}^{d_2}$. $r_1, s_1, r_2, s_2$ are some constants of the appropriate dimensions. For simplicity of exposition we assume that $d_1 = d_2 = d$. Finally, this implies that $f(\cdot, \cdot) : \mathbb{R}^d_1 \times \mathbb{R}^d_2 \rightarrow \mathbb{R}$.
% The latent parameters, $(\theta_i, \rho_j)$,  encode all information relevant to the evolution of an innings. Specifically, $\theta_i$ represents the match/innings context like the ground and weather conditions, relative strengths of the teams etc, while $\rho_j$ represents the ball-$j$ context across all innings, such as the number of balls remaining in the innings. This is a natural consequence of \textbf{Key Insight 2}, stated earlier. Note that we do not attempt to learn the latent parameters and do not need to explicitly quantify them. This is what makes the LVM such a powerful modeling tool in this setting. %Finally, we note that (\ref{eq:model4}) is a factor model, using econometric terminology, expressed as a function of the latent variables. \\
%
%If \textbf{Key Insight 1} has merit, then it implies a ``low-rank'' structure in the data. To verify its merit, we use a matrix comprising all innings in our dataset which contains over 4700 LOI innings from 1999 to 2017. The ball-by-ball data matrix has a dimensions 4700 $\times$ 300. Figure \ref{fig:singvals} shows the singular values spectrum of the top 15\% singular values (sorted in descending order) for this matrix. Note that the matrix has been normalized to re-scale all scores to remain between the range $[-1, 1]$. The plot clearly illustrates that there is ``low-rank'' structure in the data: the rank of the ``de-noised'' matrix appears to be lie within the range: $(3, 8)$. The spectrum shown is for the noisy observation matrix and the small but positive singular values can be considered noise. We note that the low-rank structure applies to the matrix of mean values generated by the function $f(\theta_i, \rho_j)$ at each $(i, j)$ index of the unobserved mean matrix. The rank-deficiency of the mean matrix helps confirm the intuition behind \textbf{Key Insight 1}. Additionally, this allows us to assume that the following linear structure exists among LOI innings:
%
%\textbf{Assumption.}  We assume that the mean, $m$, of any innings of interest, $Y$, laid out as a row vector, is a linear combination of the rows of the unobserved mean-matrix $\bM$ of the past innings. In other words, we have that:
%\begin{align} \label{eq:assumption2}
%m = \sum_{i=1}^{n} \beta_i^* m_i,
%\end{align}
%and $\beta_i^* \in \mathbb{R}$ are the \text{true} weights that allow any innings to be decomposed as a linear combination of other innings in the dataset.
%
%
%
\begin{figure}
	\centering
	\includegraphics[width=0.2\textwidth]{singular-value-spectrum.png}
	\caption{The Singular Value spectrum for all innings in the dataset (matrix of dimensions 4700 $\times$ 300. Only showing the top 15\% singular values, in descending order.}
	\label{fig:singvals}
\end{figure}
\vspace{-.1in}


%\textbf{Assumption 1.}  Our most significant modeling assumption is that $\boldsymbol{f}(\theta_i, \rho_j)$ is either (or both) of the following:
%\begin{itemize}
%\item Lipschitz in it the latent arguments;
%\item Produces a low-rank mean-matrix, $\bM$, where $\bM = [m_{ij}] = [\boldsymbol{f}(\theta_i, \rho_j)], 1 \leq i \leq n, 1 \leq j \leq b$.
%\end{itemize}
%
%It can be shown that if $\boldsymbol{f}(\theta_i, \rho_j)$ is Lipschitz, then the matrix, $\bM$, can be well-approximated by a low-rank matrix (\cite{usvt, log_rank}). \\
%
%\textbf{Assumption 2.}  We assume that the mean, $m$, of an innings of interest, $Y$, laid out as a row vector, is a linear combination of the rows of the unobserved mean-matrix $\bM$ of the past innings. In other words, we have that:
%\begin{align} \label{eq:assumption2}
%Y = m + \eps,
%\end{align}
%where $\eps$ is a row-vector of zero-mean independent noise and 
%\begin{align} \label{eq:assumption2}
%m = \sum_{i=1}^{n} \beta_i^* m_i,
%\end{align}
%and $\beta_i^* \in \mathbb{R}$.
%
%Assumptions 1 and 2 allow us to formalize the the idea in \textbf{Key Insight 1}. If there is memory in cricket innings where an innings under consideration is similar to one or more innings in the past, and such a relationship also holds across past games, then the mean-matrix of interest is rank-deficient (Assumption 1) and each innings can be considered a linear function of other innings (Assumption 2). %The linearity of the proposed relationships holds due to the low-rank assumption.



==> content/target.tex <==
\section{Target resetting} \label{sec:revised_target}

\subsection{Algorithm: Rationale \& Details} \label{sec:revised_target_algo}

\smallskip
\noindent{\bf The question.} Cricket is fundamentally an {\em asymetric} game in that team one bats for the
first half, sets the target and then second team bats to chase the target within the allocated balls. Many a 
times (around 9\% of LOIs) the game gets interrupted in the second half due to rain (and other similar events) requiring
the shortening of the game and revising the original target. Formally, let team one sets target of $t$ runs for team
two to win. Suppose team two bats for $b' < b$ of total balls and interruption happens. Now team two can
play till total of $b_1$, $b' \leq b_1 \leq b$ balls or additional $b_1 - b'$ balls. Then, what should the
target $t_1$ for team two be in $b_1$ balls? Clearly, $t_1 \leq t$. But, how much smaller?  
Specifically, there are two scenarios worth discussing: Scenario 1, when $b' = b_1$, i.e. no more play possible; and
Scenario 2, when $b' < b_1 < b$, i.e. some more play possible but not all the way. 

\smallskip
\noindent{\bf The ideal goal. } The ideal goal of the target resetting algorithm is that it 
helps counteract the impact of intervention. Put another way, by resetting the target, the outcome of the
game should be as if the game was played for the full duration with the original target. If such a goal
is achieved then the fraction of times the team batting second wins should remain the same as that when 
no intervention happens. 

\smallskip
\noindent{\bf Failure of Duckworth-Lewis-Stern (DLS).} An algorithm for target resetting is, effectively,
as essential as the rules for playing game itself. The incumbent solution adopted in
LOI cricket games is by Duckworth-Lewis-Stern \cite{dl1, dl2}. And indeed, authors in \cite{dl2} argue that 
a target resetting algorithm ought to satisfy the invariance of the fraction of time the team batting second
wins whether the intervention happens or not. 

Given that the DLS method has been used for more than a decade now, we have enough data. Specifically, we consider 1953 LOI games during the period from 2003 to 2017. From among these, 172 games were interrupted
and the DLS method was applied to reset the target / decide the winner. Among them, 59\% were won by the team
batting second. In contrast, for 1781 games that were completed without using the DLS method, the second 
batting team won 51\% of the games. Therefore, using the $\chi^2$ test of independence, we can reject the null hypothesis that 
{\em DLS does not create an advantage for team batting first or second} with the p-value of $0.048$ which is statistically
significant. Table \ref{table:dls} summarizes the data. This clearly motivates the need for a different target resetting
method. 


\begin{table}[H]
\centering
 \begin{tabular}{|| c | c | c | c ||} 
 \hline
 & Batting First Won & Batting Second Won & Total \\ [0.5ex] 
 \hline\hline
 No DLS & 865 & 916 & 1781 \\ 
 \hline
DLS  &  70 & 102 & 172 \\
 \hline
  \hline
 Total &  935 & 1018 & 1953 \\
 \hline
\end{tabular}
\caption{Contingency table for the $\chi^2$ test of independence for 1953 LOI games that produced a result. The null hypothesis is that the use of the DLS method has no effect on the distribution of games won by teams batting first or second. The p-value is 0.048 meaning that we can reject the null hypothesis.}%Games are split based on whether the team batting first or second won the game and across the games where DLS was used or not. The p-value is 0.048 and the null-hypothesis, i.e. there is no difference in distribution of games won by teams batting first or second when using the DLS method or not, can be rejected at the 5\% significance level. {\color{red} reduce this commentary, too long?} }
\label{table:dls}
\end{table}
%\vspace{-.3in}
\noindent{\bf Scenario 1: No more play.} We start with the scenario where the team batting second plays for $b' < b$
balls when the interruption happens and no more game can be played, i.e. $b_1 = b'$. The question is, what should the 
target $t_1$ be for the team batting second to have achieved at this stage to win the game?

Suppose the team batting second has made $t'$ runs losing $w'$ wickets at the intervention, $b'$. One way to decide whether the team
has won or not is to utilize forecasting algorithm proposed in Section \ref{sec:score_forecasting}. Specifically, forecast the score that team batting second will make by the end of the innings, and if it gets to the target $t$, then team batting second wins, else it loses. 

While this approach makes sense, from a cricketing perspective or setting the rule, it is has a flaw. For example, 
a good forecasting algorithm (such as ours) will forecast differently and justifiability so, depending upon {\em how} 
the state of $t'$ runs and $w'$ wickets lost is reached in $b'$ balls. Therefore, it is likely that in one scenario, team two is declared winner while in another scenario team two is declared loser even though at $b'$ balls, in both scenarios, the state of the game is identical. 

To address this, we need to come up with a forecasting algorithm that is {\em agnostic} of the trajectory leading up to the current state. Formally, we wish to estimate the score at $b'$ balls, given that target of $t$ is achieved by $b$ balls. Let $Y_{0j}$ denote the
score at ball $j$ and $W_{0j}$ denote the wicket. Then, we wish to estimate ${\mathbb E}[Y_{0b'} | Y_{0b} = t]$ and 
 ${\mathbb E}[W_{0b'} | Y_{0b} = t]$. And we wish to do so for any $b' < b$.  This estimation will not be impacted by the on-going innings or the team's performance leading up to $b'$ but instead by the collective historical data that captures the ``distribution'' of the game play. 

We propose to evaluate this using a non-parametric nearest-neighbor method. Specifically, given $n$ historical trajectories, for any $\Delta \geq 0$, let $ \mathbb{S}(t, \Delta) = \Big\{i \in [n]: Y_{ib} \in [t, t+\Delta]\Big\}.$
Then, for any $b' < b$, 
\begin{align} 
\hat{\mathbb{E}}[Y_{ib'} | Y_{ib} = t] \approx \frac{1}{|\mathbb{S}(t, \Delta)|} \sum_{i \in \mathbb{S}(t, \Delta)} Y_{ib'}. \nonumber \\
\hat{\mathbb{E}}[W_{ib'} | Y_{ib} = t] \approx \frac{1}{|\mathbb{S}(t, \Delta)|} \sum_{i \in \mathbb{S}(t, \Delta)} W_{ib'}. \label{eq:knn1}
\end{align}
This gives us ``average path to victory'' both in terms of runs scored and wickets lost. By definition, it is monotone since we are taking average of monotonic paths from actual historical innings. 

Now to compare the score of $t'$ with $w'$ wicket at $b'$ balls with this target, we have to make sure that there is a parity in terms of number of wickets lost. For example, the estimator per \eqref{eq:knn1} may suggest score of 
$\hat{t}$ with wickets $\hat{w}$ at $b'$ ball as needed for achieving target $t$ at $b$ balls. And $\hat{w} \neq w'$. Then, 
we need to {\em transform} score $\hat{t}$ with $\hat{w}$ wickets to score that is an equivalent for $w'$ wickets. Such a
transformation is not obvious at all. Next, we provide some details on the choice of such a transformation. %We propose a data-driven approach to learn such a {\em wicket resource transformation}.

\smallskip
\noindent{\bf A non-linear wicket resource transformation.}
We refer to $\boldsymbol{g}(\hat{t}, \hat{w}, \delta b', w')$ as the function needed to transform the score of $\hat{t}$ for the loss of $\hat{w}$ wickets with $\delta b' = b - b'$ balls remaining to an equivalent score for the loss of $w'$ wickets. $\boldsymbol{g}(\hat{t}, \hat{w}, \delta b', w')$ cannot be linear in terms of the wickets lost or balls remaining because the effect of wickets lost (or remaining) and balls consumed (or remaining) is not linear. For instance, the top few batters tend to play as specialist batsmen and having lost 5 out of 10 wickets means the loss of more than 50\% of the batting resources. Similarly, in a typical cricket innings teams tend to accelerate more towards the latter half of an innings meaning that at the half way mark, i.e. $b/2$ balls, teams effectively consider more than half their innings still remaining. 
$\boldsymbol{g}(\hat{t}, \hat{w}, \delta b', w')$ can be determined in two ways: parametric or non-parametric. An example of a parametric model is the DLS method which encodes information about a team's resources remaining as a function of the wickets and balls remaining. An alternate approach is to estimate the resources remaining using a non-parametric regression, e.g. random forest regression. In such a regression the wickets lost and balls remaining at each point in an innings, i.e. $w'$ and $\delta b' = b - b'$, are used as ``features'' and the percentage of target met, i.e. $t/y'$ where $y'$ is the runs scored at $b'$ balls, is the output variable. The regression model can then help complete the entire table of resources achieved (or remaining). 
In this work wee use the DLS table of resources remaining as a proxy for $\boldsymbol{g}(\hat{t}, \hat{w}, \delta b', w')$ , but with corrections. Given that we have established that the DLS method introduces a bias in favor of the chasing team, we correct the ``resources remaining'' percentages in a data-driven manner for each game. Specifically, let the target be represented by $t$,the time of interest by $b'$, the runs scored as $\hat{t}$, wickets lost as $\hat{w}$, desired number of wickets lost as $w'$, and the DLS resources remaining percentage be $d[\hat{w}][\delta b']$. Then, our correction to the DLS entry for would take the following form: $t' = \boldsymbol{g}(\hat{t}, \hat{w}, \delta b', w') = \hat{t} \cdot \big(1 - (1 - t'/t) \frac{d[w'][\delta b']}{d[\hat{w}][\delta b']} \big)^{-1}$, where $d[w'][\delta b']$ is the DLS resources remaining percentage for having lost $w'$ wickets with $\delta b' = b - b'$ balls remaining.


%The average path to victory, $A_j$, has two components: $V_j$ and $U_j$. In order to determine if the team chasing a target is on track, we cannot decide on $V_j$, average path of runs, of $U_j$, average path of wickets lost, on their own. We need to combine these two components, runs and wickets, as a function of the number of balls, $j$, to a single scaled metric to allow comparisons. This scaling is provided by the function $\boldsymbol{g}(., .)$. It maps the current state of the innings as a function of the runs made and wickets lost to the equivalent runs made if the team had used all $w_{max}$ is its wickets. This transformation can be applied to $A_j$ and the \textit{actual} trajectory taken by the chasing team to determine whether the transformed actual path was above/below the ``average scaled path to victory''. We note that $\boldsymbol{g}(., .)$ is similar to that of the DLS resources table (\cite{dl2}).  In this work, we use the publicly available standard version of the DLS resources-remaining table. Alternatives could include a data-driven approach to compute the runs scored as a fraction of the total for each runs and wickets combination across all past innings.

\smallskip
\noindent{\bf Scenario 2: Some more play.} We now consider scenario where some more play will happen, i.e. 
$b' < b_1 < b$. Assume team batting second has made $y'$ runs for the loss of $w'$ wickets at $b'$ balls. 
Using the average path to victory and non-linear resource transformation, $\boldsymbol{g}(\cdot)$, we obtain a target, say $t'$ 
for $w'$ wicket loss at $b'$ balls for achieving the eventual target of $t$. Now, we need to produce the revised target that needs
to be achieved at $b_1 < b$ balls by this team. Question is, how to do it. 

One approach is to continue using the average path to victory as before and use it to compute the 10-wicket
equivalent target at $b_1$ balls. But that is likely to be an {\em easier} target than what it should be.  The key aspect 
that needs to be incorporated in setting such revised target is what we call the target ``chasing'' mentality. In cricket 
(like most sports), it is well observed that the team plays more aggressively near the end of  the game. 
Therefore by setting end of the game closer due to $b_1 < b$, effectively we are taking the team batting second 
from their normal ``chasing mentality'' at $b'$ balls to closer to end of the 
game ``chasing mentality''. Therefore, it stands to reason that we should not simply utilize
the average path to victory which is calculated based on normal ``chasing mentality''. 

We address this challenge by simply modifying the ``average path to victory'' calculation from $b'$ to $b_1$, or
for $\delta b_1' = b_1 - b'$ balls by effectively using historical trajectories from $b- \delta b_1'$ balls to $b$ balls
rather form $b'$ to $b_1$ balls to calculate the average path to victory value at $b_1$ balls. That is, 
we find all trajectories amongst $n$ historical innings where at $b- \delta b_1'$ balls, roughly $w'$ wickets are lost.
And we use average over these trajectories and {\em stitch} it beyond $t'$ at $b'$ balls to obtain the
target at $b_1 = b' + \delta b_1'$ balls. Formally, let
\begin{align} \label{eq:end_overs_context_set}
\mathbb{T}(\delta b_1', w', t, \Delta) = \Big\{i \in \mathbb{S}(t, \Delta): W_{i (b-\delta b_1')} \in [w'-1, w'+1]\Big\}
\end{align}
Then, to reset target at $b_1 = b' + \delta b_1'$ balls starting with target of $t'$ for loss of $w'$ wickets 
at $b'$ balls, we estimate increment in target as 
\begin{align}\label{eq:end_overs_context_target}
\delta t(b_1) & = \frac{1}{|\mathbb{T}(\delta b_1', w', t, \Delta)|} \sum_{i \in \mathbb{T}(\delta b_1', w')} \big(Y_{ib} - Y_{i(b-\delta b_1')}\big). 
\end{align}
That is, the revised target is $t' + \delta t(b_1)$ at $b_1 = b' + \delta b_1'$ balls starting at revised target 
of $t'$ with $w'$ wickets at $b'$ balls. 

\smallskip
\noindent{\bf Summary of the algorithm.}

\smallskip
\noindent {\em Step 1. Average Path to Victory (Scenario 1 and 2).} 
As outlined earlier, we first determine the set of ``neighbors'', $\mathcal{S}(t, \Delta)$, referred to as $\mathcal{S}$ for simplicity. Specifically, the neighbors are all innings where the final score, $y_{ib} \geq t$. We then scale all trajectories in $\mathcal{S}$ such that they end exactly at the target, i.e. $y_{ij}^{s} = y_{ij} t / y_{ib}, \forall{i} \in \mathcal{S}$ and similarly for the wickets trajectories $w_{ij}^{s} = w_{ij} t /y_{ib} \forall{i} \in \mathcal{S}$. %We justify using the choice of neighbors and the scaling in the Appendix (Section \ref{sec:dominancescaling}). 
We then compute the average path to victory in terms of runs and wickets:
$$a_y[j] = \frac{1}{| \mathcal{S}|} \sum_{i \in \mathcal{S}} y_{ij}^{s}, \forall{j} \in [b], \quad
a_w[j] = \frac{1}{| \mathcal{S} |} \sum_{i \in \mathcal{S}} w_{ij}^{s}, \forall{j} \in [b]$$.

The $w'$ wicket equivalent target at $b'$, used in Scenario 1, is $t' = \boldsymbol{g}(a_y[b'], a_w[b'], \delta b', w')$, where $\delta b' = b - b'$ and $a_y[b'], a_w[b']$ are the average runs and wickets at $b'$.

\smallskip
\noindent {\em Step 2. Revised Target Trajectory (Scenario 2 only).} 
For Scenario 2, we now determine the revised target trajectory for the remainder of the innings, i.e. $\delta b_1' = b_1 - b'$. First, we determine the offset, which is the target, $t'$, at the point of intervention, $b'$. $t'$, the $w'$ equivalent target at $b'$, is the starting point of the revised target path. What remains is the ``stitch'' the context from the last $\delta b_1'$ of historical innings in $\mathcal{S}$ to determine the revised 10-wicket target at $b_1$. This contextual path is defined in Equations (\ref{eq:end_overs_context_set}) and (\ref{eq:end_overs_context_target}), denoted by $\delta t(b_1)$, with the $\mathcal{S}(t, \Delta)$ replaced, for simplicity, by $\mathcal{S}$, as defined in Step 1. Next, we scale this contextual path such that it never exceeds the original target, $t$. Specifically, $\delta t(b_1)^{s} = \delta t(b_1) \cdot \frac{t}{t' + \delta t(b)}$. Therefore, the revised target for each point $b_1$ where $b' \leq b_1 \leq b$ is determined by the following relationship:
\begin{align} \label{eq:revisedtarget}
t(b_1) = t' + \delta t(b_1)^{s}
\end{align} 
In the event that $t(b_1) > t$, it can be corrected to lie below $t$ for $b_1 < b$. The correction should be a function of the balls remaining, $b - b_1$, to ensure a smooth increase to $t$ in $b_1 = b$ balls.\\
\smallskip
\noindent {\em Step 3. Deciding a Winner (Scenarios 1 and 2).} 
Let the team batting second have made $y'$ runs for the loss of $w'$ wickets at the point of intervention, $b'$. For both Scenarios 1 and 2, we now have the target trajectories. In Scenario 1, the team batting second is the winner if $y' \geq t'$. In scenario 2, let the team batting second have made $y_1$ runs by the new maximum balls, $b_1$. The team batting second wins if $y_1 \geq t(b_1)$.  

In the event that in Scenario 2, there is another intervention at some point $b''$ where $b' < b'' < b_1$, and the innings is shortened even further to $b_2$ where $b'' \geq b_2 \geq b_1$, then we are back to the original Scenario 1 ($b_2 = b''$) or Scenario 2 ($b'' < b_2 < b_1$) with the maximum balls in the innings, $b$, replaced by $b_1$; the starting point moved from $0$ balls to $b'$ and the intervention point moved from $b'$ to $b''$. 

\noindent {\textbf{Fine Prints.} Some remarks are in order.

\smallskip
\noindent {\em No First-Innings Bias.}
An important feature of the algorithm is that the chasing team's target trajectory is not biased by the path taken by the team batting second. The only information from the first innings that is taken in to account is the target, $t$ in $b$ balls. How the team batting first got to their final score should not bias the target computations for the chasing team. Therefore, we take no other information from the first innings in to account.

\smallskip
\noindent{\em Neighbors.} %No Neighbors Above the Target}
We scale the ``neighbor'' target trajectories to end exactly at the target. Neighbors are those trajectories that end equal to or above the target, $t$, at the end of the innings. We justify this choice of ``neighbors'' in the Appendix (Section \ref{sec:dominance}). In rare instances, the team batting first will score an unprecedented amount of runs such that the number of past innings which end up exceeding the target are too few. In such a circumstance or any other instance where the neighbors are too few, we propose using the set of \textit{all} innings in the dataset and scaling them up/down accordingly. 

\subsection{Experiments and Evaluation} 

\smallskip
\noindent{\bf Comparison: Duckworth-Lewis-Stern.}
Given that we have established that the DLS method is biased in favor of the teams batting second (see Section \ref{sec:revised_target_algo}), the natural comparison for our algorithm is the DLS method.

\smallskip
\noindent{\bf Performance Metrics.} The metrics under consideration are those that allow to us to study the relative or absolute bias introduced by both algorithms. In Scenario 1 (as detailed next), the metric is simply the count (or proportion) of games won by the teams batting first or second with and without each of the methods. In Scenario 2 (also detailed below), we consider relative metrics which allow us to compared the relative bias of our algorithm's revised targets compared to the DLS method's revised targets.

\smallskip
\noindent{\bf Data and Setup.}
In order to evaluate the performance of any target resetting algorithm such as our method, the ideal scenario would involve a trial of the method in actual cricket games. However, this is not possible. We must, instead, rely on designing retrospective experiments and simulations which can help with evaluating the method. For all experiments discussed in this section, we use a dataset of about 230 LOI recent games which produced results and lasted longer than 45 overs in the second innings, starting in the year 2013. For the selection of the neighboring trajectories in our algorithm, we use LOI innings from the year 1999 onward. We consider the following two setups:

{\em Scenario 1}. In this experiment, we random split the candidate games in to two sets: $\mathcal{S}_A$ and $\mathcal{S}_B$. For games in $\mathcal{S}_A$, we introduce an arbitrary intervention between overs $20$ and $45$ and assume that no more play would have been possible. We ask both methods to declare a winner based on the state at the point of the arbitrary intervention. We determine the counts of teams batting first and second that are declared winners. For $\mathcal{S}_B$, we assume no interventions and determine the counts of teams batting first and second that actually won the game. Use these counts, we conduct a $\chi^2$ test of independence where the null hypothesis is that there is no difference in proportions of game won by teams batting first or second with or without the target resetting algorithm. We note the p-value and then repeat the same experiment 500 times. Under the null-hypothesis the p-value distribution ought to be uniformly distributed, by definition. 

{\em Scenario 2}. Given that we have established that the DLS method is biased in favor of the team batting second when the target is revised (Scenario 2). It is impossible to use historical data for actual LOI cricket games to retrospectively determine how the outcome might have been different had a different revised target been proposed for the chasing team. Therefore, we use the following experiment with historical data to determine whether a candidate method is poised to have any effect on the outcome of games under Scenario 2:

We introduce a hypothetical intervention, at $b' = 180$ balls (30 overs). We then assign an arbitrary revised number of overs, $b_1 = 270$ balls (45 overs). For each innings, we determine the revised remaining target runs at $b_2$ using the DLS method and our algorithm. We determine the subset of historical innings where the same number of wickets were lost at $b - (b_1 - b')$ overs as those at the intervention for the innings under consideration, i.e. $w'$. Next, we determine the proportion of innings in the subset where the revised remaining target runs were scored in the last $b - (b_1 - b')$ overs. For any method that claims to reduce the bias produced by the DLS method, we would expect the proportion of the subset of innings that achieve the revised remaining target to be \textit{lower} than that for the DLS method. 

Finally, we also determine the average percentage of the DLS revised target that our algorithm's revised targets are greater or lower than the DLS revised targets. We determine this for each over (ball) between the intervention, $b'$ and the original maximum number of overs, $b$.

\smallskip
\noindent{\bf Results.}
For the Scenario 1 experiment, where $b' = b_1$. The resulting distribution of p-values is shown in Figure \ref{fig:pvalsdls2}. We note that for our algorithm the distribution appears fairly uniform (mean = 0.49, median =0.47) while for the DLS method there is a slight bias to the left (mean = 0.41, median = 0.39). However, there is little evidence to conclude that either method suffers from an obvious bias in this scenario. This hints at the DLS method being biased under Scenario 1, similar to what was established in Section \ref{sec:revised_target_algo}.

\begin{figure}
	\centering
	\includegraphics[width=0.3\textwidth]{p-val-dist.png}
	\caption{Distribution of p-values for the bootstrapped Chi-Squared test of independence for experiments with Scenario 1.}
	\label{fig:pvalsdls2}
\end{figure}

Next, we consider the experiment for Scenario 2 where $b' < b_1 < b$, i.e. the chasing team is provided with a revised target to chase in fewer than maximum number of overs. It is impossible to use historical data for actual LOI cricket games where the DLS method was used to retrospectively determine how the outcome might have been different had a different revised target been proposed for the chasing team.  Figure \ref{fig:prop_dls_ours} shows the distribution of the differences of proportions of the subset of the historical innings that exceed the revised remaining target prescribed by our algorithm vs the DLS method. It appears to suggest that at $b_1 = 270$ balls (45 overs) when the intervention is at $b' = 180$ balls (30 overs), our algorithm's revised targets are almost always higher than those proposed by the DLS method which should reduce the bias in the favor of chasing teams experienced in LOI games. We also conduct a paired-sample t-test for the two series produced by our algorithm and the DLS method. The test rejects the null-hypothesis of the two series being the statistically the same with a p-value of $10^{-33}$.

\begin{figure}
	\centering
	\includegraphics[width=0.25\textwidth]{dls-vs-ours-proportions_final.png}
	\caption{\small Distribution of differences in proportions of historical innings that exceed the revised remaining number of runs prescribed by our algorithm vs the DLS method for over 230 recent LOI games. The mean of the differences is -3.3\% while the standard error of the mean is 0.1\%. }
	\label{fig:prop_dls_ours}
\end{figure}

Finally, Figure \ref{fig:prop_increase} shows that average upwards shift in revised targets produced by our algorithm compared to the DLS method is fairly consistent across all revised maximum durations, $b_1$, where $(b' < b_1 < b)$. The plot shows the average percentage runs that our algorithm's revised targets exceed those produced by the DLS method for all overs possible after the intervention. In this experiment, $b' = 30$ overs and $b_1$ is allowed to vary from over 31 to 49. The targets produced by both algorithms are be the same for 50 overs. The plot underscores that our algorithm should be able to reduce the bias produced by the DLS method for all revised durations. However, note that the closer $b_1$ is to the original maximum duration, $b$, the smaller the percentage increase which appeals to our intuition.

\begin{figure}
	\centering
	\includegraphics[width=0.25\textwidth]{prop_increase_over_dls2.png}
	\caption{\small The average percentage runs (with standard error bars) that our algorithm's revised targets exceed those produced by the DLS method for all overs between $b'$ and $b$.}
	\label{fig:prop_increase}
\end{figure}

\subsubsection{Case Studies}
%We present the following revised target examples on actual games using our algorithm.\\
\smallskip
\noindent{\bf Scenario 1: $b_1 = b'$ (No More Play Possible after Intervention).} We consider the game played between Pakistan and New Zealand on 01/16/2018. %Pakistan batted first and set New Zealand a competitive target of 263 in 50 overs (300 balls). 
At one stage New Zealand had lost three wickets or just 90 runs in 16 overs and 2 balls (98 balls) chasing 263. With Pakistan in the ascendency then, it took a couple of good batting partnerships from New Zealand to score the win. Figure \ref{fig:revision1} shows the resulting revised targets that New Zealand would have to make to win the game if the game stopped at any point during the innings \textit{and} no more play was possible (Scenario 1). The dotted green line is the \textit{average path to victory} while the dotted-dashed gray one is the target if the same number of wickets were lost as in the actual innings, at each point. The actual innings is shown as the solid red line. The chasing team would be declared a winner whenever the red line was above the dotted gray line. As we would expect, the red line dips below the gray line starting around the 17th over mark, signaling that Pakistan would have been declared the winners if the game stopped at that time. However, around the 38th over, New Zealand were back in the ascendency and the red line overtakes the gray line indicating that after around the 38th over if the innings stopped and no more play was possible, then New Zealand would be declared winners. The gap between the red and gray line is a proxy for how comfortably the ascendent team is ahead. These observations agree with the actual state of the game and point to a realistic target revision methodology. Note that even though the game ended at the 275th ball point, we show the trajectories for the entire 50 over (300 ball) period. 

\begin{figure}
	\centering
	\includegraphics[width=0.3\textwidth]{pak-nz-chase-revised.png}
	\caption{\small New Zealand vs Pakistan, 01/16/2018. New Zealand's actual innings (red), average path to victory (green) and revised target (dotted gray).}
	\label{fig:revision1}
\end{figure}

For another example of a famous game decided by the DLS method, please see the Appendix (Section \ref{sec:appendix_target_resetting_casestudies}).\\
\smallskip
\noindent{\bf Scenario 2: $b' = 30$ overs,  $b_1 = 45$ overs.}
Next, we consider how our algorithm would work in under Scenario 2 where the chasing team bats the first $b'$ balls assuming they will have all $b= 300$ balls (50 overs) to chase the target. However, there is an intervention at the $b'$ ball mark and only $b_1 < b$ are now possible. We use the World Cup 2011 Final between India and Sri Lanka to illustrate how our algorithm would work and its contrast to the DLS method. Figure \ref{fig:indsri_revised} shows the average path to victory in green for India when chasing the target of 275 in 50 overs (300 balls). We introduce a hypothetical intervention at the $b' = 180$ balls (30 overs) mark and assume that play will resume with a maximum of 270 balls (45 overs) possible instead of the original 300 balls (45 overs). Figure \ref{fig:indsri_revised} shows the original average path to victory (solid green line) while the dotted black line shows the targets had the revised maximum number of overs, $b_1$, been allowed to vary between $[35, 50]$. Finally, the equivalent of the black line is the dotted-dashed blue line which are the revised targets produced by the DLS method. The gap between the two methods is a feature of our algorithm. It is a consequence of taking the context of the last few overs in to account (as discussed in Section \ref{sec:revised_target_algo}) where teams can be expected to score significantly more number of runs towards the end an innings. This ``contextual'' revision of the target is what allows our algorithm to correct for the bias introduced in favor of the chasing teams by the DLS method.

%The gap between the two methods is a feature of our algorithm which corrects for the high bias in favor of the chasing team by the DLS method. It is noticeable that the revised targets produced by our algorithm expect India to reach a score very close to the original target when the revised maximum overs is close to the original maximum of $b = 300$ balls. This is an outcome of taking the context of the last few overs in to account (as discussed in Section \ref{sec:revised_target_algo}) where teams can be expected to score significantly more number of runs towards the end an innings. This ``contextual'' revision of the target is what allows our algorithm to correct for the bias introduced in favor of the chasing teams by the DLS method. %We note that in the game under consideration, India managed to overhaul the target with ease and a few balls to spare underscoring the value of taking in to account the acceleration produced by batting teams towards the tail-end of an innings. 

%Figure \ref{fig:indsri_revised} shows in blue the revised average path to victory for India. Notice how the line in blue is not parallel to the green line--this is expected because the line in blue is encoding the final 15 overs context which is comparable to the 35-50 overs on the green line. The noticeable rise in the gradient of the blue line is indicative of the last few overs mindset which would happen later if the inning was allowed its maximum 50 over (300 balls) duration. 

%The black line shows the targets had the revised maximum number of overs, $b_1$, been allowed to vary between $[35, 50]$. This is in contrast to the blue trajectory which shows the revised average path to victory once the revised maximum number of overs, $b_1$, is fixed (at 45 overs). It is no surprise then that the blue and black lines intersect at the $b_1 = 270$ balls (45 overs) mark in the situation shown in Figure \ref{fig:indsri_revised}.

%Finally, the equivalent of the black line is the one in magenta which are the revised targets produced by the DLS method. The slight upwards bias produced by our method is a feature of our algorithm which corrects for the high bias in favor of the chasing team by the DLS method. The black line gets closer to the magenta line as the revised maximum number of overs increases intersecting at the 50 overs (300 ball) mark. This makes sense because both algorithms must recover the original target if the innings was allowed to take its original maximum duration. 

\begin{figure}
	\centering
	\includegraphics[width=.35\textwidth]{ind_sri_revised_30_45.png}
	\caption{}
	\label{fig:indsri_revised}
\end{figure}
\vspace{-.1in}
%\pagebreak

%%%%%%%%%%%
%%%%%%%%%%%
\iffalse
%%%%%%%%%%%
%%%%%%%%%%%

We now turn our attention to a related problem: given the current state of the second innings in an LOI cricket game, is it possible to determine which of the two teams, the one who batted first or the one currently batting to chase the target, is in the ascendency? In cricket, the problem is of great significance. Specifically, in games where it is no longer possible to play out the maximum allocation of overs in an innings, a solution to this problem can also help declare the winner of the game. These circumstances often arise in LOI cricket games, as outlined in Section \ref{sec:revised}. As an example, consider an LOI game where the team batting second was set a target of 250 runs in 50 overs (300 balls) but experienced a rain-interruption at the half way mark (25 overs) when the score was 130 for the loss of 5 wickets. If there was no more play possible, which team should be declared a winner? If only 10 more overs were possible, instead of the originally remaining 25 overs, what should the new revised target be such that the adverse effect of the intervention, i.e. the loss of 15 overs, is nullified without leaving either of the two teams in a better or worse position than at the point of the intervention? 

One may be tempted to use the forecasting algorithm introduced earlier in this work as a means to determine which team is in the ascendency based on whether the forecasted score at the end of the innings will reach the target, or not. However, that has two short comings: (i) it is not obvious how to use the forecasting algorithm to produce target revisions in the event that the innings resumes for a shortened length; (ii) the forecasting algorithm is likely to produce different forecast estimates based on \textit{how} the chasing team got to their state at the point of the intervention which can be considered unsatisfactory and confusing by cricketers and audiences. Therefore, the goal is to produce revised targets for all possible number of remaining overs by taking in to account only the current state, i.e. runs scored and wickets lost at the point of the intervention. 

The International Cricket Council currently uses the Duckworth-Lewis-Stern (DLS) method to produce revised targets and declare a winner (\cite{dl1, dl2}) in games where one (or both) innings cannot be completed due to weather, ground conditions etc. Specifically, assume for simplicity that originally the team batting first has made $r_1$ runs in $b (=300)$ balls. This means that the chasing team has to make $t = r_1 + 1$ runs in a maximum of $b$ balls. The chasing team also has a maximum of $w$ wickets ($w = 10$). However, there is an intervention at $b_1 < b$ balls when the chasing team has made $r_b$ runs for the loss fo $w_{b_1}$ wickets. After the interruption it is only possible for the chasing team to face maximum of $b_2$ balls where $b_1 \leq b_2 \leq b$. A target resetting algorithm such as the DLS method can help with the following scenarios:
\begin{enumerate}
\item \textbf{Scenario 1: No More Play Possible ($b_1=b_2$).}\label{scenario:1} If no more play was possible after the intervention at $b_1$ balls, decide whether the chasing team can be declared to have won, or lost, the game.

\item \textbf{Scenario 2: Innings is Shortened ($b_1 < b_2 < b$)}. \label{scenario:2} An intervention occurs at $b_1$ balls where $0 \leq b_1 < b$ balls, and only $b_2$ balls are now possible in the innings, where $b_1 < b_2 < b$. The chasing team has lost $w_{b_1}$ wickets at the intervention and is still allowed to use all their remaining wickets for the shortened chase. A target resetting method must provide revised targets for each possible value of $b_2 \in \{b_1 +1, \cdots , b - 1 \}$.
\end{enumerate}

In both scenarios above, for the first $b_1$ balls the chasing team is pursuing a target of $t$ in the maximum possible $b$ balls with $w$ wickets. In scenario \ref{scenario:1}, a winner is declared taking in to account the minimum score the team is expected to have scored by the intervention ($b_1$) for the loss of $w_{b_1}$ wickets. In scenario \ref{scenario:2}, revised targets are determined that can take in to account both the wickets and new maximum number of balls remaining. As argued in Section \ref{sec:revised}, the target revision cannot be a linear function of the number of overs and wickets completed (or remaining). This is because the chasing team has the same maximum wickets $w$, for a shorted innings as it did for the original innings. Additionally, note that the loss of the first five wickets, for example, constitutes the loss of greater than 50\% of the batting resources for the batting teams. Therefore, the revised targets need to appropriately be scaled (non-linearly) to be considered equivalent. The DLS method is the incumbent and most widely adopted method to achieve this equivalence.

\subsection{Is DLS \textit{fair}?} \label{sec:fairDls}
The authors who introduced the DLS method argue in \cite{dl2} that it is \textit{fair} because the win/loss ratio between teams batting first or second is not statistically different in games that use the DLS method or not. Notably, their test was conducted on games during the early years of the DLS method. Cricketers have long felt that the DLS method appears to introduce a bias in favor of the chasing team. To put this claim to test, we perform the following experiment using actual LOI games:

We conducted a Chi-Squared Test of Independence for LOI games spanning a recent fourteen year period from 2003-2017 (inclusive). This data includes 1953 LOI games which produced a result. Our null-hypothesis was that there is no statistical difference between the proportion of games won by teams chasing with or without the application of the DLS method. Of the 1953 games in the dataset, 172 were decided based on the DLS method. Among these games, 59\% we were won by the chasing side. The remaining 1781 games were completed without using the DLS method with the chasing team's winning proportion at 51\%. Therefore, at the 5\% significance level, we have enough statistical evidence to reject the null with the p-value being 0.048. Table \ref{table:dls} summarizes these results.

This experiment allows us to statistically confirm what cricketers have felt for a while: the DLS method appears to introduce a bias in favor of the chasing team. A target resetting method must not be responsible for such a bias. In what follows, we present an alternative to the DLS method which corrects for the bias in the DLS method and is based off of the Latent Variable Model (LVM) of cricket innings introduced earlier in this work.

\begin{table}[H]
\centering
 \begin{tabular}{|| c | c | c | c ||} 
 \hline
 & Batting First Won & Batting Second Won & Total \\ [0.5ex] 
 \hline\hline
 No DLS & 865 & 916 & 1781 \\ 
 \hline
DLS  &  70 & 102 & 172 \\
 \hline
  \hline
 Total &  935 & 1018 & 1953 \\
 \hline
\end{tabular}
\caption{Contingency table for the Chi-Squared test of independence for 1953 LOI games that produced a result. Games are split based on whether the team batting first or second won the game and across the games where DLS was used or not. The p-value is 0.048 and the null-hypothesis, i.e. there is no difference in distribution of games won by teams batting first or second when using the DLS method or not, can be rejected at the 5\% significance level. }
\label{table:dls}
\end{table}


%\begin{figure}
%	\centering
%	\includegraphics[width=0.25\textwidth]{p-values-dls.png}
%	\caption{Distribution of p-values for the bootstrapped Chi-Squared test of independence across a dataset of 500 games randomly split in to games with arbitrary application of the DLS method for a random subset of games in each of the 1000 iterations.}
%	\label{fig:pvaldls}
%\end{figure}

%\subsection{A Data-Driven Model} \label{sec:data-driven-target-resetting}
%We build upon the Latent Variable Model (LVM) introduced in Section \ref{sec:model1} to propose a data-driven framework to determine revised targets. Recall that the trajectory of an innings, $Y_{ij}$, where $i$ denotes the innings and $j$ denotes the ball,  is a random realization of the following relationship:
%
%\begin{align*}
% Y_{ij} = f(\theta_i, \rho_j) + \eps_{ij},
%\end{align*}
%where $\eps_{ij}$ is zero-mean random noise with finite variance, and $f(\theta_i, \rho_j)$ is a deterministic quantity which represents the mean cumulative score, $m_{ij}$. $\theta_i$ and $\rho_j$ represent the latent variables that encode the context: $\theta_i$ represents the match/innings-specific information such as the playing conditions, venue, relative strengths of the two teams etc; $\rho_j$ represents the ball-$j$ specific context which applies to all innings in the dataset, e.g. $\rho_j = j \in \{1, 2, ... , b \}$. This LVM framework allows us the significant benefit of incorporating the all-important ``context'' in a cricket game/innings. Overhead and on-ground conditions, the relative strengths of the teams playing and other contextual information such as whether the outcome of the game has a tournament-specific consequence etc play a key role in how teams approach a cricket innings. Therefore, incorporating such context in to our model is a major advantage.

\subsection{Target Resetting as Conditional Expectation}
Recall that in Section \ref{sec:cricketmodel} we modeled the forecast for the remainder of an innings as the estimate of the conditional expectation given the past:

\begin{align*}
\mathbb{E}[Y_{ij} | Y_{ib_1},  Y_{ib_1 - 1}, ... , Y_{ib_1}], \forall{j > b_1},
\end{align*}
where $b_1$ is the point of intervention and  $b_1 < j \leq b$. However, this approach cannot be used to produce revised targets, i.e. when the duration of an innings needs to be shortened. The revised target should reflect a reasonable path to victory and not suffer from any bias from the way a team approaches its innings. It should, instead, only be a function of the final target set and the number of overs remaining in an innings. In other words, the target resetting needs to be agnostic of the team's current trajectory and the trajectory of runs in the first innings. In light of this discussion, we we view target resetting as the estimation of a different conditional expectation:

\begin{align} \label{eq:targetcondexp1}
\mathbb{E}[Y_{ij} | Y_{ib} = t],  
\end{align}
where $b_1 < j \leq b_2 \leq b$, $t$ is the target set by the team batting first, $b_1$ is the point of intervention and $b_2$ is the revised shortened duration of the innings. Unlike forecasting, (\ref{eq:targetcondexp1}) is the conditional distribution of the trajectory given a point in the future. We refer to $\mathbb{E}[Y_{ij} | Y_{ib} = t]$ as the ``average path to victory'' for the team batting second. It is effectively a trajectory which will lead the team to overhaul the target, in expectation, by the end of the full length of the innings.

\subsection{Connections to Regression} \label{sec:connection_regression}

(\ref{eq:targetcondexp1}) is akin to solving a regression problem where $Y_{ib}$ is a \textit{feature} while $Y_{ij}$ is the output variable. As in least square problems, (\ref{eq:targetcondexp1}) is the optimal solution when estimating a random variable (score at time $j$) given the model feature(s) (final score). Instead of using a parametric estimation method like least squares regression, we can use non-parametric Nearest Neighbors Regression to estimate $Y_{ij}$ conditioned on the final score. Define a set $\mathbb{S}$ as the nearest neighbors of the target trajectory. The similarity metric for $\mathbb{S}$ are all trajectories (innings) in our dataset which end \textit{near} the target, $t$. We can then use the following relationship:

\begin{align} \label{eq:knn1}
\hat{\mathbb{E}}[Y_{ij} | Y_{ib} = t] \approx \frac{1}{|\mathbb{S}|} \sum_{i \in \mathbb{S}} Y_{ij} 
\end{align}

There are several conceptual ways to compute (\ref{eq:knn1}):
\begin{enumerate}
\item \textbf{Ideally}, we would have access to limitless amount of data or could simulate limitless number of innings where the score reached by the end of the innings is exactly $t$, i.e. $Y_{ib} = t$. A sample from a set of all such innings could provide a way for us to estimate a \textit{typical} path leading to victory. However, this is unrealistic. Not only do we not have access to limitless data, we also cannot expect to use bootstrap-like approaches because our dataset might have no past innings which end at the target, $t$. 
\item \textbf{Approximate} approaches such as $k$-nearest neighbors can provide a data-driven way to generate a large enough set of innings which end up in the vicinity of the final target, $t$. However, similar to the issue stated above, our dataset might have not have a large enough number of innings which end up near the target. 
\end{enumerate}
While the ideal approach is impractical, the data-driven approximate approach provides hope. To overcome the problem of not having enough innings which end up in the vicinity of the target, we use a data-driven approach which can create the \textit{illusion} of a large enough set of candidate innings (neighbors). This approach relies on transforming a large enough set of innings by scaling all candidate trajectories such that they all end {\em exactly} at the target.  %In what follows, we propose (and justify) scaling trajectories to generate a set of approximate neighbors for the trajectory we are trying to estimate, i.e. $\hat{\mathbb{E}}[Y_{ij} | Y_{ib} = t_{i}]$. 

\subsection{Dominance Property} \label{sec:dominance}
We first note that due to the monotonicity properties of runs scored in a cricket innings, we have that if $Y_{ib} > Y_{hb}$ then $Y_{ij} \geq Y_{hj}$ in distribution for two innings $i$ and $h$ and where $j \leq b$. Similarly, if $Y_{ib} < Y_{hb}$ then $Y_{ij} \leq Y_{hj}$ in distribution. We refer to this as the \textit{dominance property} of trajectories. This property tells us that if we have a set of neighbors of the target trajectory where the final score, $Y_{ib}$, is greater (less) than the target score, $t_i$, then the estimated target trajectory for balls $j < b$ will be an upper (lower) bound on the target we are estimating. This insight allows us to detail in Appendix (Section \ref{sec:dominancescaling}) why choosing trajectories that end {\em at or above} the target and then scaling them all to end exactly at the target is the correct choice for selecting a large enough set of neighbors for each target.

%\subsubsection{Scaling Trajectories} \label{sec:scaling}
%In order to close the gap between the upper and lower bounds on the estimated target trajectories, we propose a scaling which can ensure all neighbors of the target trajectory end \textit{exactly} at the target. Such a scaling can allow us to correct for the bias introduced by using \textit{neighbors} which end above or below the target. We assume that the ratio of scores between two innings remains approximately constant across the innings. %This allows us to use a multiplicative scaling (between the final score at the end of a neighbor innings and the target score) and applying it uniformly across the entire trajectory of the neighbor innings. 
%Specifically,
%\begin{align}
%\frac{f(\theta_r, \rho_j)}{f(\theta_s, \rho_j)} \approx \frac{f(\theta_r, \rho_k)}{f(\theta_s, \rho_k)}, 
%\end{align}
%where $1 \leq r, s \leq n, 1 \leq j, k \leq b$. Recall that $n$ is the number of innings in the dataset and $b$ is the maximum number of balls allowed in an innings. This approximate equivalence will allow us to scale an innings according to its relationship with another innings. In fact, this relationship will allow us to use the \textit{same} scaling factor for every point in the innings between two innings. {\color{red} ** Will need to justify this further. **} This equivalence can be justified based on Proposition \ref{prop1} stated below.  {\color{red} ** Should also justify why the Proposition below makes some sense. **} 
%
%\begin{prop} \label{prop1}
%For an innings, let $f(\theta_i, \rho_j)$ be the mean score of for innings $i$ and at ball $j$. $\theta_i, \rho_j$ are the associated latent variables. If we have:
%\begin{align} \label{prop:assump1}
%\triangledown f_{\theta}(\theta_i, \rho_j) \approx \triangledown f_{\theta}(\theta_i, \rho_k) \frac{f(\theta_i, \rho_j)}{f(\theta_i, \rho_k},
%\end{align} then:
%\begin{align*}
%\frac{f(\theta_r, \rho_j)}{f(\theta_s, \rho_j)} \approx \frac{f(\theta_r, \rho_k)}{f(\theta_s, \rho_k)},
%\end{align*}
%where  $r$ and $s$ index two innings and $1 \leq r, s \leq n, 1 \leq j, k \leq b$.
%\end{prop} 
%
%\begin{proof} 
%Using the first-order Taylor expansion, we have:
%\begin{align} \label{eq:taylor1}
%f(\theta_r, \rho_j) \approx f(\theta_s, \rho_j) + (\theta_r - \theta_s) \triangledown f(\theta_s, \rho_j)
%\end{align}
%(\ref{eq:taylor1}) implies the following relationship:
%\begin{align} \label{eq:taylor2}
%\frac{f(\theta_r, \rho_j)}{f(\theta_s, \rho_j)} \approx 1 + \frac{(\theta_r - \theta_s)}{f(\theta_s, \rho_j)} \triangledown f(\theta_s, \rho_j)
%\end{align}
%Similar to the above, we also have that:
%\begin{align} \label{eq:taylor3}
%\frac{f(\theta_r, \rho_k)}{f(\theta_s, \rho_k)} \approx 1 + \frac{(\theta_r - \theta_s)}{f(\theta_s, \rho_k)} \triangledown f(\theta_s, \rho_k)
%\end{align}
%We now note that substituting \ref{prop:assump1} in \ref{eq:taylor2}, we get the desired relationship:
%\begin{align} \label{eq:taylor3}
%\frac{f(\theta_r, \rho_k)}{f(\theta_s, \rho_k)} \approx 1 + \frac{(\theta_r - \theta_s)}{f(\theta_s, \rho_j)} \triangledown f(\theta_s, \rho_j) = \frac{f(\theta_r, \rho_j)}{f(\theta_s, \rho_j)}
%\end{align}
%\end{proof}

\subsection{``Average Path to Victory''}
Sections \ref{sec:connection_regression} and \ref{sec:dominance} provide us with the tools to create an \textit{illusion} of a large set of approximate trajectories which can then be used to compute a \textit{typical} trajectory ending in victory, i.e. ``average path to victory'', $\hat{\mathbb{E}}[Y_{ij} | Y_{ib} = t]$. Such a path can be computed by taking the sample average of the scaled (neighbor) innings. This is akin to an approximate nearest neighbor regression where the prediction is simply the sample average of all items in a set of approximate nearest neighbors. Alternatives such as a non-uniform weighted average can also be used instead.

We note that an ``average wickets lost path'' can also be determined in an analogous manner, using the same neighboring innings but scaling each wickets lost path by the same factor as that for the runs.

\subsection{Non-Linear Transformation, g}
The ``average path to victory'' coupled with the ``average wickets lost path'' provide a prescriptive route to victory, on average. However, if the wickets lost during the innings of interest at every point during the innings are different compared to those prescribed by the ``average wickets lost path'', then we need to transform the ``average path to victory'' to reflect the equivalent runs to be scored when the exact same number of wickets are lost as that in the actual innings. As an example, imagine that in the innings of interest the chasing team has made 135 runs for the loss of 3 wickets at the 25 over mark but the prescriptive average path to victory is represented by 125 runs for the lost of 2 wickets at the same point. We need to transform the 125 runs for the loss of 2 wickets to some higher number of runs for the loss of 3 wickets so that the 135 runs actually scored can be compared directly. Further, as argued earlier in this work, such a transformation is non-linear and depends on both the number of wickets lost and the number of balls (overs) remaining. We will refer to this transformation as the function $\boldsymbol{g}(\cdot)$ which takes as its input arguments the current score, corresponding wickets lost, balls remaining and the desired wickets lost to produce a transformed score for the loss of the desired number of wickets.

%One such non-linear transformation is provided by the DLS method. The DLS method uses a table of ``resources remaining'' percentages for each possible tuple of \{wickets remaining, balls remaining\}, \cite{dl2}. However, given that we have established that the DLS method introduces a bias in favor of the chasing team, we correct the ``resources remaining'' percentages in a data-driven manner for each game. Specifically, let the target be represented by $t$, the average runs to be scored at the time of interest be $a_r$, the average wickets remaining at the time of interest be $a_w$, actual wickets lost at the time of interest be $w_r$, balls remaining be $b_r$ and the DLS resources remaining percentage be $d_{a_w}[b_r]$. Then, our correction to the DLS entry for would take the following form: $d_{w_r}'[b_r] = (1 - \frac{a_w}{t}) \cdot d_{w_r}[b_r] /d_{a_w}[b_r]$.

\subsection{Overs Remaining Context} \label{sec:oversremaningcontext}
When considering a revised maximum number of overs, $b_2$, where the intervention happens at $b_1 < b_2$ and the original maximum number of balls available were $b$, the revised average runs and wickets paths to victory must ensure that the context of the last $b - (b_2 - b_1)$ is properly accounted for. Specifically, if the intervention happens at $b_1 = 180$ balls and instead of playing the originally remaining 120 balls, the chasing team now has only 60 balls to play, the average paths to victory (both runs and wickets) must use the last 60 balls, i.e. balls in range [240, 300] to provide the new revised path to victory. Furthermore, if the chasing team had lost $s_w$ wickets at the intervention, then the ``neighbors'' used to compute the revised average path to victory must be those innings that have exceeded the target \textit{and} lost $s_w$ wickets at $b - (b_2 - b_1)$ balls. This will allow us to properly take in to account the mindset of teams when they have $b - (b_2 - b_1)$ balls left to chase a target after having lost $s_w$ wickets instead of the originally available $b - b_1$ balls and the loss of $s_w$ wickets.

\subsection{Algorithm} \label{sec:algorithm2}
Our goal is to estimate the ``average path to victory'' and scale it to produce an equivalent trajectory for the wickets lost, $w_j$, in the actual innings by ball $j$. The $w_{j}$ wicket target is necessary to provide a equivalent point of comparison to determine whether the chasing team is in the ascendency, or not, at ball $j$ of the innings.  

The inputs to the algorithm are: $y_{ij}:$ historical score trajectories in the dataset (donors); $w_{ij}:$ corresponding historical wickets lost trajectories in the dataset (donors); $t$: the original target; $b_1$: ball at intervention; $b_2$: new revised maximum number of balls; $b$: original maximum balls; $r, s$: current score and wickets lost at intervention for the innings under consideration. We also provide a non-linear transformation in the form of function $\boldsymbol{g}(\cdot)$, which transforms the current score to an equivalent score corresponding to a different number of wickets lost. $\boldsymbol{g}(\cdot)$ takes as input the the current score, the corresponding wickets lost for that score, balls remaining, and the desired wickets lost to provide an equivalent score via a non-linear transformation.  %$d_k[j]$: DLS table for $k$ wickets and $j$ ball pairs, $\zeta \in (0, 1]$: a dampening factor for the DLS correction.

Our data-driven target resetting approach is summarized in Algorithm \ref{algo3}.

\begin{algorithm}[H]
\caption{Data-Driven Target Resetting} \label{algo3}
\begin{enumerate}
\item Let $\mathcal{S} = \{i: y_{ib} \geq t\}$ and let $r_i = \frac{y_{ib}}{t} \forall{i} \in \mathcal{S}$.
\item Let $y_{ij}' = y_{ij} / r_i, \forall{i} \in \mathcal{S}$ and $w_i' = w_{ij} / r_i, \forall{i} \in \mathcal{S}$.
\item Average path to victory (runs and wickets): \\
	$a_y[j] = \frac{1}{| \mathcal{S} |} \sum_{i} y_{ij}', \forall{j} \in [b]$, \\
	$a_w[j] = \frac{1}{| \mathcal{S} |} \sum_{i} w_{ij}', \forall{j} \in [b]$.

\item Offset at Intervention: $o_y = \boldsymbol{g}(a_y[b_1], a_w[b_1], b - b_1, s)$
%\item Fraction of target met: $f[j] = a_y[j] / t, \forall{j} \in [b]$.
%\item DLS-correction: $d_{k}'[j] = \zeta \cdot (1 - f[j]) \cdot d_k[j] / d_{a_w[j]}[j] , \forall{k} \in \{0, \cdots, 10\}, \forall{j}\in [b]$.
%\item Offset: $o_y = r \cdot (1 - d_s'[b_1])/ (1 - d_{a_w[b_1]}'[b_1])$.

\item Let $\mathcal{S}_1 = \{i: i \in \mathcal{S}$, and $w_{ij} = s$ where $j = b - (b_2 - b_1) \}$.
\item Same wickets lost context:\\
	$a_y'[j] = \frac{1}{| \mathcal{S}_1 |} \sum_{i} y_{ij}', \forall{j} \in [b]$, \\
	$a_w'[j] = \frac{1}{| \mathcal{S}_1 |} \sum_{i} w_{ij}', \forall{j} \in [b]$.

\item Remaining overs context:\\
	$a_y^{''}[j] = a_y'[j] - a_y'[b - (b_2 - b_1)], \forall{j} \in [b_1, b_1 +1 \cdots , b]$, \\
	$a_w^{''}[j] = a_w'[j]- a_w'[b - (b_2 - b_1)], \forall{j} \in [b_1, b_1 +1, \cdots , b]$.

\item Another scaling based on the target: \\
	$a_y^{''}[j] = a_y^{''}[j] \cdot (a_y^{''}[b] + o_y) / t, \forall{j} \in [b_1, b_1+1, \cdots , b]$, \\
	$a_w^{''}[j] = a_w^{''}[j] \cdot (a_w^{''}[b] + s) / t, \forall{j} \in [b_1, b_1+1, \cdots , b]$.

\item Revised average path to victory, starting at offset: \\
	$\tilde{a}_y[j] = a_y^{''}[b - (b_2 - j)] + o_y, \forall{j} \in [b_1, b_1+1, \cdots , b_2]$, \\
	$\tilde{a}_w[j] = a_w^{''}[b - (b_2 - j)] + s, \forall{j} \in [b_1, b_1+1, \cdots , b_2]$.
	
\item Deciding a Winner:
	\begin{enumerate}[label=(\alph*)]
	\item Let $r_j, s_j$ be the runs scored and wickets lost by the team batting second at $b \leq j \leq b_2$. 
	\item Revised target for $s_j$ wickets lost (non-linear transformation):\\
		$\tilde{t}_j[s_j] = \boldsymbol{g}(\tilde{a}_y[j], \tilde{a}_w[j], b_2 - j, s_j)$.
		 %$\tilde{t}_j[s_j] = \tilde{a}_y[j]  (1 - d_{s_j}'[b - (b_2 - j)])/ (1 - d_{\tilde{a}_w[j]}'[b - (b_2 - j)]'), \forall{j} \in [b_1, b_1+1, \cdots , b_2]$.
	\item Chasing team wins if $r_j > \tilde{t}_j[s_j]$. Chasing team loses if $r_j < \tilde{t}_j[s_j]$. It is a tie, i.e. no-winner, otherwise.
	\end{enumerate}
\end{enumerate}
\end{algorithm}


\subsection{Algorithm Fine Print}

\subsubsection{No First-Innings Bias}
An important feature of Algorithm \ref{algo3} is that the chasing team's target trajectory is not biased by the path taken by the team batting second. The only information from the first innings that is taken in to account is the target, $t$ in $b$ balls. How the team batting first got to their final score should not bias the target computations for the chasing team. Therefore, we take no other information from the first innings in to account.

\subsubsection{Average Path to Victory}
$a_y, a_w$ are the average paths to victory which denote the average prescribed path in terms of runs and wickets lost. This should be viewed as the trajectory which, if followed exactly, would lead the chasing team to the target in exactly 50 overs (300 balls). This trajectory is simply the average of all innings in the filtered donor pool (nearest neighbors of the target). Note that this averaging relies on all innings in the donor pool to be scaled such that they reach the target in exactly 50 overs (300 balls). %This is justified by the discussion in Section \ref{sec:data-driven-target-resetting} and Proposition \ref{prop1}. 

\subsubsection{No Neighbors Above the Target}
In rare instances, the team batting first will score an unprecedented amount of runs such that the number of past innings which end up exceeding the target are too few. In such a circumstance or any other instance where the donor pool (neighbors) are too few, we propose using the set of \textit{all} innings in the dataset and scaling them up/down accordingly. We justify this recommendation in Section \ref{sec:dominancescaling}.

\subsubsection{Non-Linear Transformation, $g$}
A possible candidate for the non-linear transformation function, $\boldsymbol{g}(\cdot)$, is provided by the DLS method. The DLS method uses a table of ``resources remaining'' percentages for each possible tuple of \{wickets remaining, balls remaining\}, \cite{dl2}. We use the DLS table as a proxy for $\boldsymbol{g}(\cdot)$ , but with corrections. Given that we have established that the DLS method introduces a bias in favor of the chasing team, we correct the ``resources remaining'' percentages in a data-driven manner for each game. Specifically, let the target be represented by $t$, the average runs to be scored at the time of interest be $a_r$, the average wickets remaining at the time of interest be $a_w$, actual wickets remaining at the time of interest be $w_r$, balls remaining be $b_r$ and the DLS resources remaining percentage be $d_{a_w}[b_r]$. Then, our correction to the DLS entry for would take the following form: $\boldsymbol{g}(a_r, a_w, b_r, w_r) = \frac{a_r} {1 - (1 - \frac{a_r}{t}) \cdot d_{w_r}[b_r] /d_{a_w}[b_r]}$, where $d_{w_r}[b_r]$ is the DLS resources remaining percentage for having $w_r$ wickets and $b_r$ balls remaining.
%$d_{w_r}'[b_r] = (1 - \frac{a_w}{t}) \cdot d_{w_r}[b_r] /d_{a_w}[b_r]$. 

%\subsubsection{DLS Correction}
%We use a dampening factor, $\zeta \in (0, 1]$, when revising the DLS resources remaining table. It is the parameter that can be used to prevent our algorithm from overcorrecting the bias of the DLS method. It can be tuned using cross-validation on historical data by ensuring that in games with a single hypothetical intervention when no more play is possible, the proportion of games won by teams batting first or second remains similar to what is historically observed. 

%\subsubsection{Non-Linear Transformation, $g(. , .)$}
%The average path to victory, $A_j$, has two components: $V_j$ and $U_j$. In order to determine if the team chasing a target is on track, we cannot decide on $V_j$, average path of runs, of $U_j$, average path of wickets lost, on their own. We need to combine these two components, runs and wickets, as a function of the number of balls, $j$, to a single scaled metric to allow comparisons. This scaling is provided by the function $\boldsymbol{g}(., .)$. It maps the current state of the innings as a function of the runs made and wickets lost to the equivalent runs made if the team had used all $w_{max}$ is its wickets. This transformation can be applied to $A_j$ and the \textit{actual} trajectory taken by the chasing team to determine whether the transformed actual path was above/below the ``average scaled path to victory''. We note that $\boldsymbol{g}(., .)$ is similar to that of the DLS resources table (\cite{dl2}).  In this work, we use the publicly available standard version of the DLS resources-remaining table. Alternatives could include a data-driven approach to compute the runs scored as a fraction of the total for each runs and wickets combination across all past innings.

\subsection{Examples of Revised Targets} \label{sec:targetexamples}
We present the following revised target examples on actual games using our algorithm.
\subsubsection{Scenario 1: $b_1 = b_2$ (No More Play Possible after Intervention)}
We consider the game played between Pakistan and New Zealand on 01/16/2018. Pakistan batted first and set New Zealand a competitive target of 263 in 50 overs (300 balls). There was no intervention during the game and New Zealand was successfully able to chase the target down with 25 balls to spare for the loss of 5 wickets. However, at one stage New Zealand had lost three wickets for just 90 runs in 16 overs and 2 balls (98 balls). With Pakistan in the ascendency then, it took a couple of good batting partnerships from New Zealand to score the win. We look at the trajectory of the revised targets for the New Zealand innings. Figure \ref{fig:revision1} shows the resulting revised targets that New Zealand would have to make to win the game if the game stopped at any point during the innings \textit{and} no more play was possible (Scenario 1). The green trajectory is the \textit{average path to victory} while the dotted gray trajectory is the target if the same number of wickets were lost as in the actual innings, at each point. The actual innings is shown by the red line. For each ball, $1 \leq j \leq 300$, the chasing team would be declared a winner whenever the red line was above the dotted gray line, and no more play was possible. As we would expect, the red line lies below the gray line starting around the 17th over mark, signaling that Pakistan would have been declared the winners if the game stopped at that time. However, around the 38th over, New Zealand were back in the ascendency and the red line overtakes the gray line indicating that after around the 38th over if the innings stopped and no more play was possible, then New Zealand would be declared winners. The gap between the red and gray line is a proxy for how comfortably the ascendent team is ahead. These observations agree with the actual state of the game and point to a realistic target revision methodology. Note that even though the game ended at the 275th ball point, we show the trajectories for the entire 50 over (300 ball) period. 

\begin{figure}
	\centering
	\includegraphics[width=0.5\textwidth]{pak-nz-chase-revised.png}
	\caption{New Zealand vs Pakistan, 01/16/2018. New Zealand's actual innings (red), average path to victory (green) and revised target (dotted gray).}
	\label{fig:revision1}
\end{figure}

Next, we consider the famous World Cup 2003 game between South Africa and Sri Lanka. South Africa were chasing a target of 269 in 50 overs (300 balls). Rain made an appearance during the second innings and it became clear that at the end of the 45th over (270th ball) of the chase, no more play would be possible. Mark Boucher, a senior player in the South African team, was provided the Duckworth-Lewis-Stern (DLS) par score for the end of the 45th over and hit six runs off the penultimate ball before the intervention (anticipating play to halt at the end of the over since it had started raining). With that six, South Africa had achieved the par score and Boucher blocked the next ball for zero runs (and importantly, did not lose his wicket). South Africa walked off confident that they had achieved the DLS-revised target to win the game. However, they were informed that the ``par'' score they were provided was the DLS-revised score to \textit{tie} the game and they needed one more than par to win!  Unfortunately for South Africa, that tie meant they were knocked out of the world cup which they were also hosting in the most cruel of manners, as noted by The Guardian (\cite{dls-par-1}). 

%We use this game to illustrate how our method would work under Scenario 1. Firstly, we introduce a hypothetical intervention at the 30th over (180 balls) mark and compute the revised target and the corresponding scaled 10-wicket score by South Africa beyond the intervention.  Figure \ref{fig:saf-sri-30} illustrates that scenario. Up until that point, the team was expected to be chasing the original target of in 50 overs (300 balls). The green trajectory is the average path to victory while the red trajectory is the $w_{max} = 10$ wickets target for each point in the innings for $j > b_1 = 180$. The actual innings is shown by the black line. The trajectory in pink is the $\boldsymbol{g}(., .)$ transformed actual trajectory of the runs scored for $j > b_1 = 180$. For each ball, $b_1 < j \leq 300$, South Africa would be declared the winner whenever the pink line was above the red line, and no more play was possible. We note that after the 30 over mark, the red and pink trajectories remain very close to each other which accurately reflects the state of the chase where it was neck-and-neck after the 30th over with South Africa having lost three wickets in the space of seven overs after looking set for victory up until the 23rd over.

We also use Figure \ref{fig:saf-sri-revised} to illustrate how our method would have decided the result of the game at the \textit{actual} intervention which happened at the 45 over mark when no more play was possible. At precisely the 270 ball mark, the revised target score (for having lost 6 wickets) produced by our algorithm was 232. The score made by South Africa was 229 (for the loss of 6 wickets). Therefore, our algorithm would have declared Sri Lanka to be the winner--by a margin of two runs. This is an example that hints that the DLS method might be setting the revised target a touch too low (leading to a bias in favor of the chasing teams).

\begin{figure}
	\centering
	\includegraphics[width=0.8\textwidth]{saf-sri-chase-revised-45.png}
	\caption{Actual Intervention at 45 overs (270 balls) and no more play was possible after. New Zealand's actual innings (red), average path to victory (green) and revised target (dotted gray)}
	\label{fig:saf-sri-revised}
\end{figure}


\subsubsection{Scenario 2: $b_1 = 30$ overs,  $b_2 = 45$ overs}
Next, we consider how our algorithm would work in under Scenario 2 where the chasing team bats the first $b_1$ balls assuming they will have all $b= 300$ balls (50 overs) to chase the target. However, there is an intervention at the $b_1$ ball mark and only $b_2 < b$ are now possible. Our algorithm, like the DLS method, recommends a revised target for the chasing team. 

We use the World Cup 2011 Final between India and Sri Lanka to illustrate how our algorithm would work and its contrast to the DLS method. Figure \ref{fig:indsri_revised} shows the average path to victory in green for India when chasing the target of 275 in 50 overs (300 balls). We introduce a hypothetical intervention at the $b_1 = 180$ balls (30 overs) mark and assume that play will resume with a maximum of 270 balls (45 overs) possible instead of the original 300 balls (45 overs). Figure \ref{fig:indsri_revised} shows in blue the revised average path to victory for India. Notice how the line in blue is not parallel to the green line--this is expected because the line in blue is encoding the final 15 overs context which is comparable to the 35-50 overs on the green line. The noticeable rise in the gradient of the blue line is indicative of the last few overs mindset which would happen later if the inning was allowed its maximum 50 over (300 balls) duration. 

The black line shows the targets had the revised maximum number of overs, $b_2$, been allowed to vary between $[35, 50]$. This is in contrast to the blue trajectory which shows the revised average path to victory once the revised maximum number of overs, $b_2$, is fixed. It is no surprise then that the blue and black lines intersect at the $b_2 = 270$ balls (45 overs) mark in the situation shown in Figure \ref{fig:indsri_revised}.

Finally, the equivalent of the black line is the one in magenta which are the revised targets produced by the DLS method. The slight upwards bias produced by our method is a feature of our algorithm which corrects for the high bias in favor of the chasing team by the DLS method when choosing the offset (at the intervention). The black line gets closer to the magenta line as the revised maximum number of overs increases intersecting at the 50 overs (300 ball) mark. This makes sense because both algorithms must recover the original target if the innings was allowed to take its original maximum duration. While not always the case, we note that our algorithm tends to produce targets which lie above the DLS targets. We establish this via a statistical test in the next section.

\begin{figure}
	\centering
	\includegraphics[scale=1.5]{ind_sri_revised_30_45.png}
	\caption{}
	\label{fig:indsri_revised}
\end{figure}



\subsection{Reducing the DLS Bias} \label{sec:smallerBias}
We can use historical data to simulate and compare the performance of the DLS method and our algorithm under Scenario 1: where $b_1 = b_2$ and the innings never resumes after the intervention. Using a dataset of about 500 LOI games (starting in 2003) where the second innings lasted longer than 45 overs, we randomly partition the the dataset in to two sets: $\mathbb{S}_A$ and $\mathbb{S}_B$. $\mathbb{S}_A$ contains all games where we assume the game takes its natural course and ends without application of a target revision method. For the games in $\mathbb{S}_B$ we introduce arbitrary interventions between overs 20-45 and ask the DLS method and our algorithm to declare a winner at that stage, assuming no more play would have been possible. We then conduct a Chi-Squared test of independence using the distribution of games won by teams batting first and second for games in $\mathbb{S}_A$ and $\mathbb{S}_B$. We note the p-value and then repeat the same experiment 1000 times. The resulting distribution of p-values is shown in Figure \ref{fig:pvalsdls2}. Under the null-hypothesis the p-value distribution ought to be uniformly distributed, by definition. We note that for our algorithm the distribution appears fairly uniform while for the DLS method there is a slight bias to the left. However, there is little evidence to conclude that either method suffers from an obvious bias in this scenario.

\begin{figure}
	\centering
	\includegraphics[width=0.5\textwidth]{p-val-dist.png}
	\caption{Distribution of p-values for the bootstrapped Chi-Squared test of independence across a dataset of 500 games randomly split in to games with arbitrary application of the DLS method and our algorithm for a random subset of games in each of the 1000 iterations.}
	\label{fig:pvalsdls2}
\end{figure}

The above experiment shows that the DLS method (and our algorithm) are both unbiased in Scenario 1. However, the result of the Chi-Squared test in Section \ref{sec:fairDls} conclusively shows that a disproportionate number of teams batting second tend to win games where the DLS method is used to set a revised target. Therefore, the bias introduced by the DLS method (which we established in Section \ref{sec:fairDls}) must be coming from games in Scenario 2: where $b_2 > b_1$, i.e. the chasing team is provided with an actual revised target to chase in fewer than maximum number of overs. It is impossible to use historical data for actual LOI cricket games where the DLS method was used to retrospectively determine how the outcome might have been different had a different revised target been proposed for the chasing team.  Therefore, we use the following experiment with historical data to show that our algorithm is poised to reduce the bias in favor of the chasing teams that the DLS method suffers from.

We use hundreds of innings in our dataset and introduce a hypothetical intervention, at $b_1 = 180$ balls (30 overs). We then assign an arbitrary revised number of overs, $b_2 = 270$ balls (45 overs). For each innings, we determine the revised remaining target runs at $b_2$ using the DLS method and our algorithm. We also determine the subset of historical innings where the same number of wickets were lost at $b - (b_2 - b_1)$ overs as those at the intervention for the innings under consideration. We then determine the proportion of innings in the subset where the revised remaining target runs were scored in the last $b - (b_2 - b_1)$ overs. For any method that claims to reduce the bias produced by the DLS method, we would expect the proportion of the subset of innings that achieve the revised remaining target to be \textit{lower} than that for the DLS method. 

Figure \ref{fig:prop_dls_ours} shows the distribution of the differences of proportions of the subset of the historical innings that exceed the revised remaining target prescribed by our algorithm vs the DLS method. The experiment was performed over 230 LOI games from the past few years. The mean of the differences is approximately -1\%. This appears to suggest that at $b_2 = 270$ balls (45 overs) when the intervention is at $b_1 = 180$ balls (30 overs), our algorithm's revised targets are higher, on average, than those proposed by the DLS method which should reduce the bias in the favor of chasing teams experienced in LOI games. We also conduct a paired-sample t-test for the two series produced by our algorithm and the DLS method. The test rejects the null-hypothesis of the two series being the statistically the same with a p-value of $10^{-6}$.


\begin{figure}
	\centering
	\includegraphics[width=0.7\textwidth]{dls-vs-ours-proportions.png}
	\caption{Distribution of differences in proportions of historical innings that exceed the revised remaining number of runs prescribed by our algorithm vs the DLS method for over 230 LOI games. The mean of the differences is -1\% while the standard error of the mean is 0.01\%. }
	\label{fig:prop_dls_ours}
\end{figure}

Finally, Figure \ref{fig:prop_increase} shows, using the same innings as those used for the experiment summarized in Figure \ref{fig:prop_dls_ours}, that average upwards bias in revised targets produced by our algorithm compared to the DLS method is fairly consistent across all revised maximum durations, $b_2$, where $(b_1 < b_2 < b)$. The plot shows the average percentage runs that our algorithm's revised targets exceed those produced by the DLS method for all overs possible after the intervention. In this experiment, $b_1 = 30$ overs and $b_2$ is allowed to vary from over 31 to 49. The targets produced by both algorithms must be the same for 50 overs. The plot underscores that our algorithm should be able to reduce the bias produced by the DLS method for all revised durations. However, note that the closer $b_2$ is to the original maximum duration, $b$, the smaller the percentage increase which appeals to our intuition.

\begin{figure}
	\centering
	\includegraphics[width=0.7\textwidth]{prop_increase_over_dls.png}
	\caption{The average percentage runs that our algorithm's revised targets exceed those produced by the DLS method across all possible revised new maximum duration (overs) of the innings ($b_2 \in \{31, 32, \cdots , 49\}$) after the intervention $b_1 = 30$ overs. We introduce an arbitrary intervention at the 30 over mark and determine the revised targets for the DLS method and our algorithm. The bars show average percentage increases for each over are calculated over 250 recent games.}
	\label{fig:prop_increase}
\end{figure}

%%%%%%%%%%%
%%%%%%%%%%%
\fi
%%%%%%%%%%%
%%%%%%%%%%%

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../cricket"
%%% End:


==> content/terminology.tex <==
\section{Cricket: Setting and Terminology} \label{sec:setting}

We use this space to describe concretely the basics of the game of cricket relevant to the rest of this work. We consider the limited-overs international (LOI) format of the game: a LOI game is played between two teams, each of whom gets to bat once. Each team's turn to bat is referred to as an {\em innings}. Therefore, each LOI game is two-innings long.  Each innings is allocated a maximum number of times that a ball can be bowled (similar to pitching in baseball) to the batters. A single such bowling event is called a {\em ball}. Six consecutive balls are referred to as an {\em over}. In this work we consider LOI games which mandate that an innings can last a maximum of 300 balls or, equivalently, 50 overs. The team batting second, also referred to as the {\em chasing} team, needs to make one more run than the team batting first to win the game.

The total runs scored by a team is the cumulative sum of the runs scored on each of the {\em balls} in the innings. Both teams get a maximum of 10 {\em wickets} they can lose in an innings. The loss of a {\em wicket} is an important event in an innings: it signifies the event where a batter is declared {\em out} and is not allowed to play further role in the innings (as a batter). The loss of ten wickets means the team has no batters left to contribute to the innings. Therefore, an innings can end if maximum overs are bowled or ten wickets are lost, whichever happens earlier. As an example, in the ICC Cricket World Cup Final in 2015, New Zealand batted first and lost all ten wickets for a cumulative score of 183 in 45 overs (270 balls). Australia were set a target of 184 in a maximum of 50 overs but they chased it successfully in 33 overs and 1 ball (199 balls) for the loss of only 3 wickets.

It is worth emphasizing that individuals comprising a team cannot change between innings. Everyone on the team can get to bat but only a few typically bowl. The consequence of this is that a team typically comprises several specialists: some playing primarily as batters, some primarily as bowlers with a few who are called upon to do both. Normally teams send their specialist batters to bat ahead of the bowling specialists. This implies that the batting strength of a team degrades non-linearly, i.e. a loss of five wickets implies much more than 50\% of the batting strength exhausted.

\subsection{Reduced Innings: Revised Targets} \label{sec:revised}
A 50 over (300 ball) game of two innings can last about 8 hours. Often, weather conditions such as rain can prevent a game from lasting the entire 100 overs across two innings. This leads to several scenarios of interest to this work. One such scenario happens when the intervention, e.g. rain, happens at some point during the second innings. While the target was set for a maximum of 50 overs (300 balls) and 10 wickets, it may not be possible to play the maximum number of overs. In such a situation, the target for the chasing team needs to be revised to reflect an equivalent target for the new reduced maximum number of overs. However, note that the chasing team is still allowed access to all 10 of their wickets. As discussed earlier, since the batting capabilities do not scale linearly with the number of wickets, the target revision cannot be done in a simple linear manner. For example, if the team batting second was chasing 250 runs in 50 overs and can now only play a maximum of 25 overs, a revised target of 125 would not be considered equivalent, or {\em fair}, because the chasing team still gets to use all 10 of their wickets meaning that they have a shorter period (25 overs) over which to spend the same number of batting resources (10 wickets). Much of this work aims to address the problem of target resetting in reduced innings.
